REBAR: Retrieval-Based Reconstruction for Time-series Contrastive Learning

The success of self-supervised contrastive learning hinges on identifying positive data pairs, such that when they are pushed together in embedding space, the space encodes useful information for subsequent downstream tasks. Constructing positive pairs is non-trivial as the pairing must be similar enough to reflect a shared semantic meaning, but different enough to capture within-class variation. Classical approaches in vision use augmentations to exploit well-established invariances to construct positive pairs, but invariances in the time-series domain are much less obvious. In our work, we propose a novel method of using a learned measure for identifying positive pairs. Our Retrieval-Based Reconstruction (REBAR) measure measures the similarity between two sequences as the reconstruction error that results from reconstructing one sequence with retrieved information from the other. Then, if the two sequences have high REBAR similarity, we label them as a positive pair. Through validation experiments, we show that the REBAR error is a predictor of mutual class membership. Once integrated into a contrastive learning framework, our REBAR method learns an embedding that achieves state-of-the-art performance on downstream tasks across various modalities.

==> scatchwork.tex <==
% \mxnote{i am a bit nervous about saying contrastive learning is sota, bc new sota is masked autoencoder}
% Other approaches have existed, exploiting stationarity, using a time stamp specific, including frequency information, for limited success. <--- do i want to start beef?
% Self-supervised contrastive learning typically uses invariances within the data to identify positive data pairs to push together in the embedding space and negative data pairs to push apart to learn a rich and generalizable representations without labels. However, within the time-series domain, identifying pairs is non-trivial, augmentations are typically used to create a positive pairing, but depending on the augmentation it may 
% The key component in the success of self-supervised contrastive learning is the ability to identify positive data pairs to push together in the representation space that share semantic meaning. \textbf{}
% Self-supervised contrastive learning uses the inherent structures and invariances found within the data to design augmentations to constructive positive pairings, which are then used as psuedo-labels for 
% has had a significant impact in the computer vision, leading to significant improvements across , spurring the development of new model architectures and innovation of , but has not found comparable wide-spread success in the time-series domain. 


In computer vision, there is a range of established, meaningful\textcolor{red}{meaningful is a wishy washy word} invariances \textcolor{red}{need citations}to leverage for constructing positive pairs, but in time-series, the augmentations are simple and limited \textcolor{red}{again, simple and limited sound wishy washy as used}(e.g. cropping and masking)\textcolor{red}{need citations}. In this paper, we introduce Between-Sequence Retrieval Reconstruction error as a proxy for predicting class membership in a contrastive learning framework. Intuitively, if we can borrow information from time-series A to reconstruct missing gaps found in time-series B, we hypothesize that time-series A and B will have similar latent generative states\textcolor{red}{representations?} and thus have similar downstream classification labels. We use a transformer-based architecture to match temporal information between two different time-series sequences for reconstruction, and show that the ensuing reconstruction error provides a strong metric for unsupervisedly\textcolor{red}{this isn't a word} learning a representation that achieves state-of-the-art performance in downstream classification tests.\textcolor{red}{describe the class, potentially give citations for the datasets}

 While successful in computer vision\textcolor{red}{ and NLP?}, it has not found widespread success in time series.
Self-supervised learning uses the inherent structures and invariances found within the data to learn a generalizable representation without labels, and it has found great success across many domains, but noticeably, hasn't become widely adopted within the time-series space. To understand this, for In self-supervised contrastive learning, computer vision has a wide-range of meaningful invariances to leverage for constructing positive pairings, unlike in time-series, which is typically limited to simple augmentations, such as cropping and masking. To this end, we introduce the novel idea of utilizing Between-Sequence Retrieval Reconstruction error as a proxy for predicting class membership within a contrastive learning framework. Intuitively, if we can borrow information from time-series A to reconstruct missing gaps found in time-series B, we hypothesize that time-series A and B will have similar latent generative states and thus have similar downstream classification labels. We use a transformer-based architecture to match temporal information between two different time-series sequences for reconstruction, and show that the ensuing reconstruction error provides a strong metric for unsupervisedly learning a representation that achieves state-of-the-art performance in downstream classification tests.


Contrastive learning is a promising self-supervised representation learning technique, particularly within computer vision. It pushes positive pairs closer within latent space and negative pairs further apart.  Positive pairs are formed through complementary views of the same instance: thus the success of contrastive learning strongly depends on the data augmentation used. In vision, augmentations are designed to learn well-understood invariances within instances and promote within-class alignment between instances. Time series are less interpretable than images: the augmentation choices are thus less obvious. Instead of augmenting, we hypothesize that if a time-series can successfully borrow generative information from a different time-series for a masked reconstruction task, this pairing would constitute a positive pairing within a contrastive learning framework. This allows for learning a representation useful for both forecasting and classification. This leads to us doing masked reconstruction with auxiliary samples. We demonstrate state-of-the-art results with this approach. 

In time series, complex, time-varying properties make the augmentation choice less obvious. 

Self-supervised learning uses the underlying structures found within the data to learn a rich and generalizable representation without labels, and has enabled fine-tuning on a various of downstream tasks, de-emphasizing the necessity of large labeled datasets. This has lead to breakthroughs in fields such as the computer vision domain with the introduction of architectures like SimCLR \citep{chen2020simclr}, MoCo \citep{he2020moco}, Masked Autoencoder \citep{he2022mae} and the natural language processing domain with architectures like BERT \citep{devlin2018bert}. Self-supervised learning is particularly valuable for time-series, in which high-frequency sensors can be set up autonomously and continuously collect large amounts of unlabeled data or in the case of medical time-series such as electrocardiogram signals, annotation has a high cost due to the necessitation of medical expertise. However, self-supervised learning approaches have yet to find comparable widespread and revolutionary success in our time-series field. 

Self-supervised learning uses the underlying structures found within the data to learn a rich and generalizable representation without labels, and has enabled fine-tuning on a various of downstream tasks, de-emphasizing the necessity of large labeled datasets. 



% similiarity under reconstruction MSE measure is a good proxy for mutual class membership

if we can borrow information from the temporal structures in A


use a retrieval-based method to look at temporal structures in A that most closely match the temporal structures 


for constructing comparisons across instances.

From the best of our knowledge, no one has done this before

Self-supervised learning uses the underlying structures found within the data to learn a rich and generalizable representation without labels, and has enabled fine-tuning on a various of downstream tasks, de-emphasizing the necessity of large labeled datasets. 

One of the most prominent methods of self-supervised learning is contrastive learning, which works by creating "meaningful" positive and negatives pairs of data instances, such that when the positive pair is drawn together in the embedding space and negative pair apart, this embedding space captures semantic relationships between data and thus can be easily used for fine-tuning downstream tasks, such as classification. 

SimCLR was the original work to introduce the power of contrastive learning  \cite{chen2020simclr}, and since then, there have been multiple breakthoughs in this field with the introduction 

This has lead to breakthroughs in the computer vision domain with the introduction of architectures MoCo \citep{he2020moco}, and SimSiam \cite{chen2021simsiam}, which demonstrated
. 


However, each of these architectural developments were developed within the computer vision field, where augmentations are straightforward. 

Masked Autoencoder \citep{he2022mae} and the natural language processing domain with architectures like BERT \citep{devlin2018bert}. Self-supervised learning is particularly valuable for time-series, in which high-frequency sensors can be set up autonomously and continuously collect large amounts of unlabeled data or in the case of medical time-series such as electrocardiogram signals, annotation has a high cost due to the necessitation of medical expertise. However, self-supervised learning approaches have yet to find comparable widespread and revolutionary success in our time-series field. 



has seen broad success within the computer vision domain \citep{he2020moco, chen2020simclr} and




This technique is straightforward and intuitive in the vision space: there is a wide-range of augmentations that exploit the well-established invariances found within photos that can be used to generate a positive image from the original anchor image. However, augmentations in time-series are simple and limited, as many augmentations risk fundamentally changing the time-series (e.g. a scaling augmentation on ECG data can easily change the diagnosis from healthy to unhealthy). TS2Vec \citep{yue2022ts2vec} is a contrastive learning method for time-series and uses two simple augmentations, cropping and masking, to form positive pairs, and in fact found that the utilizing of additional augmentations, such as jittering and scaling, led to performance drops. Time-Frequency Consistency \citep{zhang2022tfc} then actually uses jittering and scaling, along with time-shifting and cropping, but also introduces the use of augmentations in the frequency domain in order to achieve strong performance. Our approach utilizes an innovative novel approach for constructing comparisons across instances.

\begin{align*}
    - \log \frac{\exp(\textrm{sim}(z_a, z_p)/ \tau)}{\exp(\textrm{sim}(z_a, z_p)/ \tau) + \sum_{n \in N} \exp(\textrm{sim}(z_a, z_n)/ \tau)}
\end{align*}

We do this and that. in this paper we did these




broke performacne


As mentioned earlier, they assume the time
series data to follow some invariant assumptions which do
not hold for diverse and ever-changing distributions of time
series


positive pairs closer within latent space and negative pairs further apart.  Positive pairs are formed through complementary views of the same instance: thus the success of contrastive learning strongly depends on the data augmentation used. 




works by pushing and is quite straightforward in the vision domain, as positive pairings are easily achieved by 

but augmentations in time-series are simple and limited. Ts2vec only uses masking and cropping, and focuses on learning by exploiting consistency. TFC is very innovative and introduces augmentstion in the frequency domain, after finding that augmentations in only time-series domain is useless. TNC attempts to avoid this augmentation thing completely by relying on a stationarity assumption and sampling neigh, but in practice runs very slowly achieves subpar results. 


, specifically

This such approach is particularly valuable to time-series data. which can be 

, significantly reducing the need for labeled samples and 


advancing the capabilities of AI across diverse tasks, leading to breakthroughs in various fields like computer vision, natural language processing, and more.


Self-supervised learning uses the inherent structures and invariances found within the data to learn a generalizable representation without labels, and it has found great success across many domains, but noticeably, hasn't become widely adopted within the time-series space.


Time series data is crucial as it provides valuable insights into patterns, trends, and dependencies over time, and 



In particular, it would be super useful for time-series data










\textcolor{red}{Way too general, the last phrase will get the reviewer ready to reject and they will simply be looking for a good kill shot.}
Time series data is crucial as it provides valuable insights into patterns, trends, and dependencies over time, and in doing so, each series is very specifically designed to capture particular phenomena, ranging from electrical activity of the heart in electrocardiogram (ECG) signals to stock prices in the financial market. As such, how the most salient information is interpreted is variable and differs greatly by domain: for example, in ECG signals, frequency information is essential for diagnosing irregular heart rhythms and whereas in financial time series, the trend is more valuable. Furthering this comparison, we note that certain time series, such as ECG, were handcrafted to evaluate specific systems and necessitate interpretation by trained professionals, whereas others, such as financial time series, are nebulous by design. 

With the advent of machine learning, we have seen the development of deep learning architectures that are able to perform a variety of tasks on time series data, such as forecasting, classification, and imputation. However, in general, we often see this field lag behind others, such as computer vision and natural language processing. Time series data is distinctedly different, each time point has the dense information present in an individual pixel, while also having temporal dependencies present in the interaction of words within a sentence. 


Self-supervised learning and by extension, contrastive learning, has shown itself as a way to leverage large sets of unlabeled data to learn representations for downstream tasks. In the time-series field, this is a natural fit, with many the time-series data originating from always-on sensors that are continuously collecting data and especially in regards to the large amounts of medical time-series, most of them are unlabeled, due to a large portion of signals solely being used for monitoring purposes and because labeling is an expensive effort requiring expert annotation. 


leverage unlabeled data 

. In a field as populated as medical data with continously monitoring signals, such an idea is critically important, yet there are very few works that have researched this in detail, and even fewer that attempt




, we have seen success in development of such architectures that can perform well regardless of domain, like this and that. However, noteably, although we see the field move towards self-supervised learning as a way to leverage unlabeled data or as a representation learning method to 

The field has not unified behind a given approach. 

With this context, it is difficult to develop a generalized approach towards 


medical time-series needing to be interpreted by trained professionals (e.g. ECG) and others, such as financial time-series are nebulous by design.




Time-series data is a critical type of data, used to describe many differnet modalities, from. This data is collected very precisely through sensors, designed to specifically measure some sort of phenomenom. Due to this, a lot of information may be too specific, if we do not fully understand the phenomon , which means if we understand it, then its 

In particular, augmentation-based methods 

\textcolor{red}{Results: what version of your results would lead to different reject/accept outcomes, assuming the rest of the paper was good.}


Metric learning is a machine learning paradigm focused on either using or learning a suitable similarity function (i.e. metric) between data points in either a supervised or unsupervised  fashion. Log-ratio Loss uses continuous labels with a contrastive learning approach in an supervised image retrieval task by enforcing the distance ratios in the label space to be preserved in the learned embedding space \citep{kim2019metricbeyondlogratio}. Proxy Anchor Loss is a loss function designed to learn a metric for supervised image classification \citep{kim2020metricproxy}.  RINCE \citep{hoffmann2022metricrince} uses a ranked list of positives, which originate from class label hierarchies or time-differences in a video, to iteratively add the positive pairs into the negative set in the NT-Xent loss function's denominator for an approximation of relationships between positives. ROC \citep{kan2021metricroc} jointly learns a feature embedding function and a metric function that respects the relative order of k-means clusters of the feature embeddings. Each of these methods present are tied to the computer vision space, but they provide interesting ideas for avenues of future research for our method, in which we could use the REBAR metric as a continuous label, rather than as a discrete one, to contrast examples or have a joint learning strategy between the metric and the feature embedding function. 
Metric learning is a machine learning paradigm focused on either using or learning a suitable similarity function (i.e. metric) between data points in either a supervised or unsupervised  fashion. Log-ratio Loss uses continuous labels with a contrastive learning approach in an supervised image retrieval task by enforcing the distance ratios in the label space to be preserved in the learned embedding space \citep{kim2019metricbeyondlogratio}. Proxy Anchor Loss is a loss function designed to learn a metric for supervised image classification \citep{kim2020metricproxy}.  RINCE \citep{hoffmann2022metricrince} uses a ranked list of positives, which originate from class label hierarchies or time-differences in a video, to iteratively add the positive pairs into the negative set in the NT-Xent loss function's denominator for an approximation of relationships between positives. ROC \citep{kan2021metricroc} jointly learns a feature embedding function and a metric function that respects the relative order of k-means clusters of the feature embeddings. Each of these methods present are tied to the computer vision space, but they provide interesting ideas for avenues of future research for our method, in which we could use the REBAR metric as a continuous label, rather than as a discrete one, to contrast examples or have a joint learning strategy between the metric and the feature embedding function. 

Time series representation learning methods generally falls under two different categories, those focused on capturing global context between time-series and those focused on capturing local context within time-series.\textcolor{red}{does context have a formal definition? If not, is there a more technical word?}


Combining a denoising objective and a DTW-based triplet similarity discrimination was shown to be useful as a pre-training task, but their approach is only evaluated on global time-series classification tasks\textcolor{red}{what does this refer to? What is an example of a local classification task? Per time point classification? Forecasting?}. Time-Frequency Consistency modeling improves upon this by proposing augmentation banks\textcolor{red}{what are augmentation banks? Briefly summarize.} to explicitly capture invariances across the time and frequency domain for a generalizable pre-training approach \citep{zhang2022tfc}. However, this method is again designed for capturing global information for entire time-series, rather than those that require local context within a time-series (e.g. subsequence classification, forecasting\textcolor{red}{these examples should be earlier}).

For capturing local context, a simple triplet loss based approach has been proposed, in which positive subsequences are sampled as a smaller subset of the reference subsequence and the negative subsequence are sampled from a different time-series to learn subseries consistency  

\citep{Franceschi2019simpletriplet}. TS2Vec utilizes relatively simple augmentation techniques (i.e. cropping with overlap and time-point-wise masking augmentation techniques) to generate positive examples, and thus may be unable to capture more complex temporal invariances, such as frequency information \citep{yue2022ts2vec}.



% The key component in the success of self-supervised contrastive learning is the ability to identify meaningful positive data pairs, such that when they are pushed together in the embedding space, the embedding will encode information useful for downstream tasks. This construction of the positive pair is typically done through augmentations that exploit the inherent structures and invariances present in the data, allowing us to create another view of the original instance, while preserving semantic meaning. However, for time-series, constructing positive pairs is non-trivial, as augmentations may break temporal dependencies (e.g. shuffling) or the semantic meaning present (e.g. flips).  In this paper, we introduce a novel approach for identifying meaningful positive pairs of time-series: the retrieval-based reconstruction metric. Intuitively, if we can borrow information from time-series A to accurately reconstruct masked values in time-series B, we hypothesize that time-series A and B will have similar temporal structures and thus have similar downstream classification labels. We use a convolutional transformer to match temporal information between two different time-series sequences for reconstruction, and show that the ensuing REtrieval-BAsed Reconstruction (REBAR) error provides a strong metric for learning a representation that achieves state-of-the-art performance in downstream tasks.

% SSL is really powerful and the key component in its succes
% Key to the success of self-supervised contrastive learning is the ability to identify meaningful positive data pairs such that when pushed together in embedding space, the embedding will encode information useful for downstream tasks. This construction of the positive pair is typically done through augmentations that exploit the inherent structures and invariances present in the data, allowing us to create another view of the original instance, while preserving semantic meaning. However, for time-series, constructing positive pairs is non-trivial, as augmentations may break temporal dependencies (e.g. shuffling) or the semantic meaning present (e.g. flips).  In this paper, we introduce a novel approach for identifying meaningful positive pairs of time-series: the retrieval-based reconstruction metric. Intuitively, if we can borrow information from time-series A to accurately reconstruct masked values in time-series B, we hypothesize that time-series A and B will have similar temporal structures and thus have similar downstream classification labels. We use a convolutional transformer to match temporal information between two different time-series sequences for reconstruction, and show that the ensuing REtrieval-BAsed Reconstruction (REBAR) error provides a strong metric for learning a representation that achieves state-of-the-art performance in downstream tasks.
% make this last sentence clearer

Self-supervised learning uses the underlying structures found within the data to learn a rich and generalizable representation without labels, and has enabled fine-tuning on various of downstream tasks, de-emphasizing the necessity of large labeled datasets. This has led to breakthroughs in fields such as the computer vision domain with the introduction of architectures such as SimCLR \citep{chen2020simclr}, SimSiam \citep{chen2021simsiam}, Masked Autoencoder \citep{he2022mae} and the natural language processing domain with architectures such as BERT \citep{devlin2018bert}. Self-supervised learning is particularly valuable for time series, in which high-frequency sensors can be set up to autonomously and continuously collect large amounts of unlabeled data, or in the case of medical time series, such as electrocardiogram signals, annotation has a high cost due to the necessitation of medical expertise. However, our time-series domain presents itself as a unique challenges, with each time-point having the sparse information present in an individual pixel in an image, while also having the temporal dependencies found in the interaction of words in a sentence. 

Self-supervised learning uses inherent structures within data to learn a rich and generalizable representation without labels. It thus enables improved fine-tuning on various downstream tasks, reducing the need for large labeled datasets. This has led to breakthroughs in computer vision with architectures such as SimCLR \citep{chen2020simclr}, SimSiam \citep{chen2021simsiam}, and Masked Autoencoder \citep{he2022mae}, and in natural language processing with architectures such as BERT \citep{devlin2018bert}. It is particularly beneficial for time series, where high-frequency sensors can autonomously collect large volumes of unlabeled data, or in medical time series such as electrocardiogram signals where annotation is costly due to the need for medical expertise. However, time-series data presents unique challenges due to the sparse information at each time point, similar to an individual pixel in an image, and the temporal dependencies akin to word interactions in a sentence.

 From a subject's long time-series, we sample 1 anchor time-series and 1 candidate time-series from each class. After reconstructing the masked-out anchor time-series as the query with each candidate time-series as the key, the class for the anchor time-series is predicted to be the class of the comparison time-series which provided the best REBAR error. 

 Before utilizing it in a contrastive learning framework, we must evaluate whether our REBAR error is a good predictor for mutual class membership by borrowing the downstream classification labels in a validation experiment. Our data is structured such that for a given subject, they have a long, dynamic time-series signal in which the classification label changes over time (e.g. a subject's PPG signal which fluctuates based on their fluctuating stress states), and with this, we utilize a within-subject, class balanced sampling method. From a subject's long time-series, we sample 1 anchor time-series and 1 candidate time-series from each class. After reconstructing the masked-out anchor time-series as the query with each candidate time-series as the key, the class for the anchor time-series is predicted to be the class of the comparison time-series which provided the best REBAR error. Results are shown below in Figure


Before applying it in a contrastive learning framework, we must evaluate whether our REBAR error is a good predictor for mutual class membership by borrowing the downstream classification labels in a validation experiment. First, we sample 1 anchor time-series and 1 candidate time-series from each class. After reconstructing the masked-out anchor time-series as the query with each candidate time-series as the key, the class for the anchor time-series is predicted to be the class of the comparison time-series which provided the best REBAR error. Then the results can be visualized with a confusion matrix and with an accuracy metric.  


% maybe push this into appendix, which is validated with our results in table, which is validated in our 
% With this validation procedure, we can better understand our masking procedure in which an extended mask is used during training but a transient mask is used during application. 

% and compare different methods for masking. We explore two different masking methodologies: an extended mask, where continuous chunk of a signal is masked out, or a transient mask,  where a select percentage of time stamps is masked out at random.



visualize our results from this validation procedure 


validation procedure allows us to precisely understand how REBAR is a good proxy for predicting mutual class membership. 


Figure \ref{fig:validationtswithattn}




shows it with some specific examples and then the confusion matrix 
This figure also helps demonstrate how our REBAR model reconstructs the query using keys with different class labels. 



, but the class that the one it pertained to achieved the best performance. 

Then the results can be visualized with a confusion matrix and with an accuracy metric.  

In order to train the REBAR model, there are two main different masking strategies. An "extended" mask strategy involves masking out a continuous chunk of a signal, and a "transient" mask strategy is where a select percentage of time stamps are independently masked out at random. In order to 



Our data is structured such that for a given subject, they have a long, dynamic time-series signal in which the classification label changes over time (e.g. a subject's PPG signal which fluctuates based on their fluctuating stress states), and with this, we utilize a within-subject, class balanced sampling method. 


Results are shown below in Figure


Two different sampling strategies and two different masking strategies


to only from the key input timeseries, as the information to directly reconstruct the query is exactly found in the key, because they are the same time-series. 

. This is done so th
Then during validation, when the query and key inputs are different time-series, the model searches for the most reelvant informaation in the key to retrieve information from 

Therefore, our strategy is to train a model 

it to the data all the same, thus leading to a model that sucks ass. 




the model is fitting to keys that shouldnt be able to reconstruct the signal


especially in this unsupervised learning scenario in which labels are unknown.


we cannot train a model to retrieve 




Therefore, during training, the query and key input time-series are the same, with difference being that the query input time-series is masked out. This is done so th


In order to train the REBAR model, there are two main different masking strategies. An "extended" mask strategy involves masking out a continuous chunk of a signal, and a "transient" mask strategy is where a select percentage of time stamps are independently masked out at random. In order to 
, and this is confirmed in our ablation results % empirical findings
% involves masking out a select percentage of the time stamps at random.  


time stamps are dropped out at random 
we could follow a "transient" mask strategy


The first is with s a transient masking strategy  


As such, in order to train our REBAR model to we utilize a large receptive field to learn how to fill in missingness in  to teach the model how to look for relevant structures for reconstruction, before 
still agle to capturfe



 meaningfully compare two timepoints in a time-series, it is necessary to utilize the local signal context around the queries and keys. This can be accomplished via convolutional self-attention \citep{convattn}, which models the query and key function as a convolution, which we demonstrate for $f_q$ below:
 


% Therefore, if we can remove all residual connections from the original query input, this means that the reconstruction of the query input is solely and completely the result of transformations on regions of the key input. Thus




then the expected value formulation


and then utilize only these identified regions in a function 

% directly use such regions in a function 
. Specifically, given a query input time-series with masked out values, a separate key input time-series 

the key input based on how they match with regions in the query we would like to reconstruct

Specifically, given 


time points in the query we would liek to reconstruct 

. This retrieval mechanism can be modeled as an attention mechanism, in which we would like to 

We claim that the pair-wise comparisons in the transformer's self-attention module are an attractive method for modeling the quasiperiodic dependency structure of pulsative signals.



The idea behind REBAR is finding a way to understand how when retrieving
We would like to understand how closely two time-series are related through 


with REBAR. 


selfattention is a good fit because of this, we 

remove residual connections


Our REBAR method uses a modified version of the Bottleneck Dilated Convolutional transformer architecture proposed in PulseImpute \citep{xu2022pulseimpute} to retrieve information from a time-series to reconstruct the masked values found in a query time-series, which can be seen in Figure \ref{fig:rebarmodel}. The model is kept simple to ensure that actual temporal structures. The crux of the model comes down the self-attention module, which is described below


we keep it simple as possible to ensure actual temporal structures are compared





the dilated convs are similar to scale, and they allow us to capture large receptive field. Rather expectedly, when trained  we allow the model to "overfit" 

PulseImpute originally utilized this mechanism for a self-supervised imputation task in self-attention mode, such that the query and key time-series are the same, to retrieve temporal structures within the same sequence for reconstruction and demonstrated through attention visualizations that this model was able to attend to similar temporal structures as the query's missing temporal structures. 

\textbf{Metric Learning}
Metric learning is a machine learning task that can either focus on using a metric between data points \textcolor{red}{don't you \textit{learn} a metric?}, to learn a representation useful for another related task, or on learning this metric to describe similarities between data points, and here we focus on the first paradigm for our use-case for representation learning. Our approach of using the REBAR metric to guide contrastive learning is somewhat similar to other metric learning approaches, but these other approaches are typically not self-supervised and their metrics are typically derived from labels in a supervised learning task. Log-ratio Loss uses continuous labels with a contrastive learning approach in an supervised image retrieval task by enforcing the distance ratios in the label space to be preserved in the learned embedding space \citep{kim2019metricbeyondlogratio}. RINCE \citep{hoffmann2022metricrince} uses a ranked list of positives, which originate from class label hierarchies or time-differences in a video, to iteratively add the positive pairs into the negative set in the NT-Xent loss function's denominator for an approximation of relationships between positives. ROUL \citep{kan2021metricroc} jointly learns a feature embedding function that respects metric order consistency and a metric function that respects relative order of k-means clusters of the feature embeddings, building off of the DeepCluster \citep{caron2018deepcluster} approach. Each of these methods present are tied to the computer vision space, but they provide interesting ideas for avenues of future research for our method, in which we could use the REBAR metric as a continuous label, rather than as a discrete one, to contrast examples or have a joint learning strategy between the metric and the feature embedding function. \textcolor{red}{it's not entirely clear how relevant some of these are to what you're doing, other than future work. In which case they probably belong at the end.}


The invariances present within images are well-understood (e.g. flipping, rotating), and as such, augmentations are designed around these invariances allow for an image and an augmented version of that same image to retain it's original semantic meaning, thus forming a positive pair. 

However, in time-series, such invariances are not as well-understood or generalizable, and as such, augmentations in time-series are simple and limited, as many augmentations risk fundamentally changing the time-series' semantic meaning (e.g. scaling ECG data may change the diagnosis) or destroy the temporal dependencies present (e.g. shuffling).



Our novel approach is designed around the unique temporal properties found within time-series and utilizes a retrieval-based reconstruction metric to identify positive and negative pairs in a contrastive learning framework. The intuition of how it works is as follows: given query time-series B with masked out values, if we can successfully retrieve matching temporal structures in key time-series A in order to reconstruct B, then this implies that time-series A and B share similar temporal structures, and we hypothesize that they will then also have similar downstream classification labels. 


We implement this retrieval-based reconstruction with a convolutional cross-attention model  that trains with self-attention to learn how to retrieve temporal structures for reconstructing masks, and switches to cross-attention to evaluate retrieval-based reconstruction across two different time-series. 
Our innovative method, known as REBAR (REtrieval-BAsed Reconstruction), harnesses this insight and convincingly establishes its suitability as a proxy for mutual class membership even before its application within a contrastive learning framework. Then, once we use REBAR as a positive/negative labeler in a contrastive learning setting, we demonstrate that our method is able to achieve state-of-the-art results on downstream classification tasks on multiple time-series datasets across a variety of data types. 

We design our REBAR model with a convolutional cross-attention architecture that learns how to retrieve temporal structures between differing time-series to effectively evaluate how a time-series can be reconstructed using only temporal information

% "We design our REBAR model with a convolutional cross-attention architecture that learns how to retrieve relevant temporal structures from distinct time-series, enabling effective reconstruction of one time-series using another."

% We design our REBAR model with a convolutional cross-attention architecture that, given time-series A, learns how to retrieve the most relevant temporal structures from a different time-series, time-series B, and uses only these temporal structures from time-series B to reconstruct the masks in time-series A. to reconstruct one of them, and does so with a map 

Our REBAR model is designed to reconstruct one masked time-series through transformations of a different time-series. The masked time-series serving solely to identify the most relevant regions within the other time-series

Our rebar model is designed to reconstruct a masked time-series completely from a different time-series as the input, with the masked time-series only being used to identify what regions in the other time-series are the most relevant.

based only on a different time-series does



We designed our REBAR model as a mapping from an input time-series to a reconstruction for a different masked out time-series, by identifying the most relevant information in the input time-series in a cross-attention comparison between the two time-series

Our rebar model identifies the regions in an un-masked time-series that would be most useful for reconstructing a different masked out time-series. Then, using these identified regions in the un-masked time-series, we learn a map from the un-masked time-series to the reconstruction of the other, different masked time-series

This reconstruction is based only on a different time-series, the only information from the query is being used to identify what regions in the key time-series could be useful for its own reconstruction

with a map from these identified regions, to the reconstruction


retrieve temporal structures between differing time-series to effectively evaluate how a time-series can be reconstructed using only temporal information



retrieve temporal structures for reconstructing masks, and switches to cross-attention to evaluate retrieval-based reconstruction across two different time-series.



Our hypothesis is that if one time-series is useful for reconstructing another, then they should form positive examples, thus l


can be shared between time-series to aid in reconstruction. 



Our novel approach is designed around the unique temporal properties found within time-series and utilizes a retrieval-based reconstruction metric to identify positive and negative pairs in a contrastive learning framework. The intuition of how it works is as follows: given query time-series B with masked out values, if we can successfully retrieve matching temporal structures in key time-series A in order to reconstruct B, then this implies that time-series A and B share similar temporal structures, and we hypothesize that they will then also have similar downstream classification labels. 


% We implement this retrieval-based reconstruction with a convolutional cross-attention model  that trains with self-attention to learn how to retrieve temporal structures for reconstructing masks, and switches to cross-attention to evaluate retrieval-based reconstruction across two different time-series. 

% \textcolor{red}{this implies is a strong statement. We initially hypothesize, and then given that it helps with prediction, it lends additional support. We want to weaken this implies, but not by too much.}


% Before utilizing retrieval-based reconstruction for contrastive learning, we show that it is a good predictor for mutual class membership, through various validation experiments and visualizations. Then, with this relationship established, we then assert that A and B would serve as a good positive pairing and use our retrieval-based reconstruction as a metric to construct positive and negative pairings for contrastive learning framework, and achieve state-of-the-art results on downstream classification tasks on multiple time-series datasets across a variety of data types compared to other time-series self-supervised learning approaches. 
we begin by saying how outline related work with other ssl methods in time-series and other retrieval-based methods in other domains. then we explain our method architecture, validation, and usage within contrastive learning. finally we present our results and discuss avenues for future work

\textcolor{red}{the two paragraphs above could likely be one and shorter.}

TS2Vec \citep{yue2022ts2vec} uses a hierarchical contrasting method to learn representations at the timestamp level and creates positive examples with two simple augmentations, cropping and masking. They found that utilizing additional augmentations, such as jittering and scaling, led to performance drops. In contrast to this, TF-C \citep{zhang2022tfc} explicitly includes jittering and scaling augmentations, along with the cropping and time-shifting augmentations, but also utilizes frequency-based augmentation for a frequency-based encoder. TS-TCC \citep{eldele2023tstcc} uses dual-augmentation to create a positive pair, with one "weak" augmentation, with jittering and scaling, and a "strong" augmentation, with jittering and permutation. As we discussed earlier, the permutation augmentation breaks temporal dependencies present in the time-series, and scaling can easily change the semantic meaning of a bounded signal, but nevertheless, each of these papers utilized these augmentation strategies due to their validation in individual empirical ablation studies. 



CoST \citep{woo2022cost} uses scaling, shifting, jittering, for time-series forecasting, 

BTSF \citep{yang2022btsf} uses time-stamp masking to be better than jittering, Rotation, Scaling, Magnitude Warping, Permutation, Slicing, Time Warping, Window Warping, SPAWNER, (wDBA), Random Guided Warping (RGW) and Discriminative Guided Warping (DGW), and  found that  for classification, forecasting and anomaly detection

TimeCLR \citep{yang2022timeclr} uses a learned DTW-based augmentation for classifcation

CLoCs \citep{kiyasseh2021clocs} says stuff next to each other or acrtoss leads are positive

CLUDA \citep{ozyurt2022cluda} uses masking and jittering for classification

SSLAP \citep{lee2022SSLAPP} uses masking for classification


include CoST \citep{woo2022cost} which used scaling, shifting, jittering, BTSF \citep{yang2022btsf}, which used timestamp masking, TimeCLR \citep{yang2022timeclr}, which used a learned DTW-based augmentation, and CLUDA \citep{ozyurt2022cluda}, which used masking and jittering. The difference in augmentation strategies across each of these methods demonstrate the inconsistency of augmentations across different methods, thus we seek to utilize a sampling-based approach with our REBAR method.




CoST \citep{woo2022cost} uses scaling, shifting, jittering, for time-series forecasting, 

BTSF \citep{yang2022btsf} uses time-stamp masking to be better than jittering, Rotation, Scaling, Magnitude Warping, Permutation, Slicing, Time Warping, Window Warping, SPAWNER, (wDBA), Random Guided Warping (RGW) and Discriminative Guided Warping (DGW), and  found that  for classification, forecasting and anomaly detection

TimeCLR \citep{yang2022timeclr} uses a learned DTW-based augmentation for classifcation

CLoCs \citep{kiyasseh2021clocs} says stuff next to each other or acrtoss leads are positive

CLUDA \citep{ozyurt2022cluda} uses masking and jittering for classification

SSLAP \citep{lee2022SSLAPP} uses masking for classification

\begin{align*}
    O(T  ((12(nobs/100)^{1/4}) ^2 &= O(T  ((12(T/100)^{1/4}) ^2)) \\
    &= O(T^{3/2}) \textrm{ per ADF calculation} \\
    O(CT^{3/2}) & \textrm{ per ADF calculation per channel} \\
    O(C(T^{3/2} + (2T^{3/2}) + (3T^{3/2}) )) & \textrm{ per ADF calculation per channel if we scale it up 3 times} \\
    O(N \cdot S! \cdot C \cdot T^{3/2}) & \textrm{ per ADF calculation per channel if we scale it up S times}
\end{align*}
\citep{}

and does not well-characterize why 

. Additionally, TNC addresses the unlabeled example with a




positive subsequences in a stationary region around the anchor subsequence from the origin sequence and samples unlabeled (rather than negative) subsequences from the non-neighboring region \citep{tonekaboni2021tnc}. However, their method relies on a heuristic hyperparameter to debias the unlabeled instance from the loss function, and it depends on the Augmented Dickey-Fuller statistical stationarity test in the determination of temporal neighborhoods, which leads to a slow run-time and does not characterize precisely why stationarity is important for discriminative power, which is a bigger problem now that other methods have surpassed its performance. 


tyhis paper uses retrieval as a way of evaluating
Re
retrieving the data from the database, based on the query provided by user or application

. These methods rely on the idea of retrieving relevant items or documents from a pool of candidates, often using similarity measures, ranking algorithms, or indexing structures. Retrieval-based methods are used in various applications, including:


These methods rely on the idea of retrieving relevant items or documents from a pool of candidates, often using similarity measures, ranking algorithms, or indexing structures.


Retrieval-Enhanced Transformer \citep{borgeaud2022retro}, while having a similar naming scheme, does not use the transformer for retrieval, unlike our approach. Instead, they use a kNN method to retrieve the most relevant documents to the transformer encoder. 

% Despite its similarity in name, Retrieval Transformer \citep{borgeaud2022retro}
% there are other ssl methods that focus on learning aimputation based methods or are generative models, but generally, this is not what we are aiming for. but we are focusing on generalizable embeddings

"To our knowledge, we are the first to employ a retrieval-based approach for self-supervised learning in time-series data. While some self-supervised time-series learning works employ retrieval as an evaluation method for their representations (Chen et al., 2021; Zhu et al., 2020), our innovation lies in the integration of retrieval within our method rather than solely as an evaluation technique."

be used in a "cross" fashion to assess and synthesize information across two different sequences. 

to reconstruct masked values in another time-series, and this retrieval process should be able to reflect how similar the temporal structures are across the two time-series.

Therefore, if we remove all residual connections from the query input \textcolor{red}{why do this? I don't get it. Equations would help.}, this shows that this REBAR cross-attention network is a map of the key input to the output reconstruction, and thus, the quality of the reconstruction allows us to understand how much information the key input shares with the masked out query input.\textcolor{red}{there is too much going on in this paragraph: it's pretty hard to understand. Does this correspond to one of your pictures?}



When we use cross-attention to compare two different time-series, 

because we dont want any positional information, bc we want to borrow based on retrieve information based upon similarity of temporal structures within the subsequences, and not on the position

we want to cmopare how similar temporal structures are across time-series and not want our model to learn how to recnostruct based on position. the position is also not very useful when we eventually use this cross-attention to compare across 
so that our cross-attention mechanism can more effectively compare , and only relative neighborhood information is important, because 

and the retrieval function learns a pure similarity function 


utilize the approach suggested by the Bottleneck Dilated Convolutional transformer architecture proposed in PulseImpute \citep{xu2022pulseimpute} to capture a larger receptive field, while learning the conditional probability of the keys given the query.




This is especially problematic  

in order to do an effective retrieval in time-series, we need to compare the temporal structures around query and keys, instead of a single time-point, as each time-point is quite sparse in information and does not have the same semantic content as a word. Thus, $f_{k/q}$






 % and the transformation of the keys, $f_v( \textbf{x}_{k})$, being used to reconstruct a masked out query. 

 

, and as such, the query time-series not directly used 

emphasis is magnified by how the query time-series is not directly used for reconstruction, it is only 


 
Now we note that the query time-series is not directly used for this reconstruction, being only present in 


: it is only used to identify regions in the key time-series to retrieve with $p(\textbf{x}_k | \textbf{x}_q)$. 


The attention mechanism allows us to identify relevant regions in the key time-series that would aid reconstruction in a different query time-series with masked out values with $p(\textbf{x}_k | \textbf{x}_q)$. Then, the module utilizes these identified regions \textcolor{red}{needs math notation}in the key time-series and processes them through the neural network to reconstruct the masked out points \textcolor{red}{math notation} with $f_v( \textbf{x}_{k})$. 

However, in order to do so, the vanilla cross-attention mechanism can only compare single timepoints between time-series with its choice of $f_{k/q}(\cdot)$\textcolor{red}{need to make it clear why this is bad}, so in order to have a meaningful comparison within the attention mechanism, it is necessary to utilize the local context around the queries and keys. Therefore, we utilize the approach suggested by the Bottleneck Dilated Convolutional transformer architecture proposed in PulseImpute \citep{xu2022pulseimpute} to capture a larger receptive field, while learning the conditional probability of the keys given the query. In order to handle the masks, we utilize the partial convolution architecture \citep{liu2018partialconv}, which ignore the calculation at masked time-points. In order to to address distribution shift across our input time-series\textcolor{red}{what kinds of distribution shifts? Why are they a problem/do we need to address them?}, we utilize a simple reversible instance norm\textcolor{red}{how does this help?}, normalized to the query input \citep{kim2021revin}. The linear layer following the cross-attention layer mimics the projection layer in the originally proposed cross-attention block \citep{vaswani2017attnisallyouneedtransformer}, and as alluded to previously, we remove the residual connection from the query input, to ensure that the output reconstruction does not directly use any temporal structure information in the query for reconstruction. The full architecture is illustrated in Figure \ref{fig:rebarmodel}. \textcolor{red}{again this is super confusing, we need to work on it.}

we can freeze our REBAR model \textcolor{red}{again, we need math notation for the model/terms that we're freezing}and utilize a differing query and key input time-series\textcolor{red}{need equations for the different time series that we're using}. The model will now have learned to retrieve the most relevant regions \textcolor{red}{would help if we had an equation/math notation for these regions}in the key time-series based on the masked regions \textcolor{red}{math notation for the masked regions} in the query and attempt to use them to reconstruct the masks, and the resulting reconstruction error is our REBAR metric to compare in our contrastive learning process. This process is further detailed in the Section \ref{fig:rebarapply}, and it is illustrated in Figure \ref{fig:rebarapply}a).




The anchor time-series is “labeled” as the comparison time-series’ class which provided the best retrieval-based reconstruction with the masked-out anchor time-series 


We find the monte carlo expectation of predicting class labels with 

 to understand how a lower REBAR error between two time-series correlates to mutual class membership.

 
in a class-balanced comparison approach

Due to the strong diagonal, prominent across all 3 datasets, we show that REBAR is able to 
Confusion Matrices demonstrating how REBAR is a predictor of mutual class membership. Before its use in contrastive learning, REBAR's effectiveness in identifying pos/neg examples can be evaluated by leveraging downstream classification labels. Given an anchor time-series, we sample a candidate time-series from each class. The anchor time-series is predicted to be the class of the candidate that provided the lowest REBAR error with a masked-out anchor. The Monte Carlo expectation of this is shown in the confusion matrices. The strong diagonal pattern observed across all three datasets highlights REBAR's capability in predicting mutual class membership. 


% "For instance, our aim is to train a model that retrieves complete heartbeats for ECG signal reconstruction. This way, reconstructing a normal signal from one with irregular heartbeats will result in a higher reconstruction error than reconstructing from another normal signal. However, if the model is only trained to reconstruct transient trends, like short upward lines, both normal and abnormal signals will exhibit these trends, leading to similar performance in a retrieval-based model and thereby reducing its discriminative capability."


%expression


% For example, we would like to learn a model that retrieves an entire heartbeat for ECG signal reconstruction, so that reconstructing from a signal with misshapen heartbeats versus regular ones will result in distinctly different reconstruction errors.

Then, given a normal ECG signal, a signal with misshapen heartbeats would have a higher error when reconstructing it than the error incurred from using a different normal signal to it. 


If instead, the model was only learned to reconstruct transient trends, such as short upwards line, both normal and abnormal signals will have this trend, and a retrieval-based model would perform equally as well, thus removing any discriminative power based on Reconstruction error.

"For instance, our goal is to train a model that retrieves complete heartbeats for ECG signal reconstruction. In this scenario, a signal with irregular heartbeats should exhibit a higher reconstruction error when attempting to reconstruct a normal signal, compared to the error incurred when reconstructing another normal signal. However, if the model is trained solely to reconstruct transient trends, like short upward lines, both normal and abnormal signals will feature these trends. Consequently, a retrieval-based model would perform similarly on both signal types, thereby diminishing its discriminative power based on reconstruction error."


another normal ECG signal as the key, then it can reconstruct the original normal signal well, but 


, so that if we use another normal ECG signal, $\textbf{X}_2$,  it will be able to reconstruct the original well, but if we use an unhealthy ECG signal with mishappen heart beats, the REBAR model attempts to reconstruct with the unhealthy signal's mishappen heart beats. 


econstruction is poor. If we learn a model that only reconstructs transient trends, such as a brief upwards line,  both healthy and unhealthy ECG signals will have these brief upwards line present, so a retrieval-based reconstruction method would perform well on both of them, making them not very distinguishable. 


ecg we would like to retrieve an entire heartbeat, therefore, there is a big difference in reconstruction when we reconstruct a signal from a healthy heartbeat versus an unhealthy one.


For example,  we would like the model to retrieve entire heartbeats from a signal, so that when used for recnostruction, we could have a better error for a signal that borrowed a healthy heart beat to reconstruct a healthy heartbeat, versus a signal that donated a 



retrieve the heartbeats from other signals to reconstruct a signal 


would like the model to learn how to capture temporal structures that are characteristic of the downstream labels associated with time-series. For example, within an ECG signal, we would like to capture a misshapen heartbeat signal and identify other signals that have similar misshapen heartbeats that can help reconstruct this temporal structure. Conversely, signals with normal heartbeats will incorrectly reconstruct the signal with a normal heartbeat, and thus be identified with a higher reconstruction error. 

 


we can see that even with the transient mask, the REBAR model maintains a sparse attention.


an intermittent mask is useful because it masks out time-points throughout the entire signal and because we need to reconstruct at each one of these, this allows us to evaluate the retrieval function at each one of them.
The model is still trained to retrieve large temporal structures, but the intermittent mask during the application phase allows us to evaluate temporal structures throughout the query time-series. In Figure \ref{fig:validationtswithattn}, we can see that even with the transient mask, the REBAR model maintains a sparse attention. 




allows us to evaluate the similarity between the two subsequences and label them as positive or negative. Then, with this, we can learn an embedding space 


acts as a positive/negative labelers, depending on how well 


as a positive/negative labeler.
in order to label 
First we use By using a cross-attention mechanism to learn how to retrieve temporal structures between differing time-series to effectively evaluate how one time-series can be used to reconstruct another, and use this to guide a contrastive learning approach that learns a class discriminative representation space. We compare REBAR to other contrastive learning approaches and demonstrate its capability to 


achieve state-of-the-art results within a contrastive learning framework in downstream classification tasks across diverse data types.

. Then, if this holds true, then these two subsequences should be positive examples 

This borrowing of information for reconstruction idea is captured with our REtrieval-BAsed Reconstruction model, in which 




Intuitively, if we can borrow information from time-series A to reconstruct missing gaps found in time-series B, we hypothesize that time-series A and B will have similar latent generative states\textcolor{red}{representations?} and thus have similar downstream classification labels.

similar latent generative states and thus have similar downstream classification labels.


Next, recognizing that

Thus, given 



% Each subsequence has a specific classification label, and this label tells us the state of the latent generative state generated 

% how the temporal pattern


% a common paradigm is using a sensor to continously collect a signal over a long time-period. this signal is evolving.
% Thus we refers to this extended signal as the "full" time-series. 
% a common challenge involves crafting tasks from long, extended time-series datasets. Particularly when these extended time-series capture evolving dynamic states (such as changing activity labels), the approach is to partition the time-series into shorter subsequences and assign labels to each subsequence. 



% in which each subsequence is an instantiation of a latent generative state described by its classification label. This is especially true for biophysical health signals: for example, an active accelerometer sensor attached to a user outputs a single "extended" time-series over the course of a day. However, throughout the day, the user engages in various activities, such as walking and sitting, which generates different temporal patterns captured in the subsequences. 

% With this understanding, we hypothesize that if we can borrow information from one subsequence to successfully reconstruct the missing gaps in a different subsequence, then the two subsequences may share similar latent generative states and downstream classification labels, and thus should be considered to be a positive pair. We investigate this hypothesis and harness this insight with our REtrieval-BAsed Reconstruction (REBAR) method. In REBAR, a cross-attention model retrieves information from one subsequence to reconstruct another, and the ensuing reconstruction error is a metric to evaluate the similarity between the two, allowing us to identify positive and negative pairs to train our contrastive learning model to learn a class discriminative representation space.


% To the best of our knowledge, our idea of using retrieval-reconstruction as a metric for contrastive learning is completely novel, even outside of time-series.

We would like our REBAR error to act as a quasi-distance metric between two time-series $d(\textbf{X}_q,\textbf{X}_k)&=\Vert\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)-X_q\Vert_2^2$ and also capture information about their downstream classification labels. When two time-series have a low REBAR error, then they also share classification labels (i.e. if $d(\textbf{X}_q,\textbf{X}_k)$ is small, then $y(\textbf{X}_q ) = y(\textbf{X}_k)$, where $y(\textbf{X})$ is the true class label of $\textbf{X}$). If this holds, then when training our contrastive learning method to pull pairs of data points with low REBAR error together, it would also effectively group points of the same classes together.


to capture information useful for downstream tasks, such as classification, so that when two time-series have a low REBAR error, they also share classification labels (i.e. if $\Vert\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)-X_q\Vert_2^2$ is small, then $y(\textbf{X}_q ) = y(\textbf{X}_k)$,


Our REBAR error is a quasi-distance metric between two time-series, and it is defined as
\begin{align*}
    d(\textbf{X}_q,\textbf{X}_k)&=\Vert\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)-X_q\Vert_2^2
\end{align*}


We would like, $ d(\textbf{X}_q,\textbf{X}_k)$ to capture information useful for downstream tasks.


% \amnote{
% \textcolor{red}{REBAR's error is like a distance. If two points are close then } The goal of REBAR is to help us learn to pull pairs of data points with the same class label closer together in embedding space, and with different class labels further apart.  
% \begin{itemize}
%     \item Intuition
%     \item Pre-contrastive stage
%     \item Contrastive learning stage
% \end{itemize}
% }
% \textcolor{red}{Because the method is pretty involved, you should give a high-level summary without equations of the entire training/applying rebar approach before you delve into details, particularly because you're using equations.}




% During training, the lack of positional encoding prevents the model from learning to reconstruct based on absolute position

% given $\textbf{X}_q \neq \textbf{X}_k$,
% In order to use our REBAR model, it will need to have learned how to retrieve relevant information from the key input to reconstruct in masked query $\bar{\textbf{x}}_q$ with $p(\textbf{x}_k | \bar{\textbf{x}}_q)$, such that
%, and for this quasi-distance to have the property that when sequences are close according to our quasi-distance, then those sequences are likely to have the same label. 


We would like to use REBAR to form a quasi-distance metric: we will use this quasi-distance to form positive and negative pairs. Points that are close together will be positive pairs, and those further apart will be negative pairs. We use the following quasi-distance:

While this is not a valid distance (depending on REBAR it may violate symmetry and the triangle inequality), and is actually random due to masking, we would like it to approximately exhibit \textit{some} of the properties of a distance: specifically that the distance between a point (sequence) to itself is (approximately) zero, and positivity: that the distance between two distinct points is always positive. Positivity is very likely to hold, as we would need perfect reconstruction for it not to. However, we can train $\textrm{REBAR}$ to approximate the first condition.

% REBAR metric to capture information useful for downstream tasks, such as classification, so that when two time-series have a low REBAR error, they also share classification labels (i.e. if $\Vert\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)-X_q\Vert_2^2$ is small, then $y(\textbf{X}_q ) = y(\textbf{X}_k)$, where $y(\textbf{X})$ is the true class label of $\textbf{X}$). If this holds, then when training our contrastive learning method to pull pairs of data points\amnote{we should make it clear what we mean. Make embeddings close to each other?} with low REBAR error together, it would also effectively group points of the same classes together. In the pre-contrastive learning stage, we train REBAR to retrieve information for reconstruction, then in the contrastive learning stage, we apply REBAR to evaluate how information can be retrieved between two differing time-series to estimate mutual class membership. 

% so that the embedding space 

% two time-series have a low REBAR error, then ideally it implies that they share classification labels:
% \textcolor{red}{If we're going to use an equation here, we should describe it in words first and then say 'More formally,'}
% Let
% \begin{align*}
%     \hat{X}_q&=\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k).
% \end{align*}
% We posit that 
% that is, if $\Vert\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)-X_q\Vert_2^2$ is small, then $y(\textbf{X}_q ) = y(\textbf{X}_k)$,
% \textcolor{red}{the next equation looks super heuristic. I wil rewrite it.}
% \begin{align*}
%     \textrm{Ideally, } \textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k) \textrm{ accuracy }\uparrow \implies y(\textbf{X}_q ) = y(\textbf{X}_k)
% \end{align*}
% where $y(\textbf{X})$ is the true class label of $\textbf{X}$. 

%, we still train $\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)$ in an unsupervised fashion, and we do not have $y(\cdot)$. Therefore, given a random $\bar{\textbf{X}}_q, {\textbf{X}}_k$ pair, it is unclear whether we want to minimize or maximize $\Vert\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)-\textbf{X}_q\Vert_2^2$. So,
Specifically, in the \textit{pre-contrastive learning stage} we
% it is unclear whether we want the model to learn a good reconstruction with a given random $\bar{\textbf{X}}_q, {\textbf{X}}_k$ pair with $y(\textbf{X}_q ) \stackrel{?}{=} y(\textbf{X}_k)$.
% \amnote{how do we know whether we want $X_k$ to properly reconstruction $X_q$?}
% , but the optimizer still tries to attempts to fit to the reconstruction, regardless of whether the query and key actually share class labels, $y(\textbf{X}_q ) \stackrel{?}{=} y(\textbf{X}_k)$. 
\begin{align*}
    \textrm{Train\ \ } \textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k) \textrm{\ \ with\ \ } \textbf{X}_q  = \textbf{X}_k.
\end{align*}
Then as long as REBAR can learn to approximately reconstruct a masked signal using the full version of the signal, $d$ will have the distance between a point and itself be approximately $0$. Now, what is of particular interest is how the trained model can be used in the contrastive learning setting, in which $\textbf{X}_q  \neq \textbf{X}_k$. 

% Because $y(\textbf{X}_q ) = y(\textbf{X}_k)$ when $\textbf{X}_q  = \textbf{X}_k$. The key has exactly the information that the query is missing, so we expect for our model to learn how to exactly retrieve the matching region in the key and reconstruct. Now, what is of particular interest is how the trained model can be used in the contrastive learning setting, in which $\textbf{X}_q  \neq \textbf{X}_k$. 
%  The key has the query's exact masked-out information, so we expect for our model to learn how to retrieve the exact information from the key. 
% Then, given a trained model, we are interested in applying the model in a setting in which the key and query are different, in order 


% , but we also hypothesize that a learned model will still be able to retrieve the most relevant region, even when the key and the query are different.

%, but what is more significant, is how this trained model performs in the contrastive learning setting in which the keys and queries are different and the key does not have exact . 
% when it tries to retrieve a matching region, when the matching region does not exist. 

% model will be able to exactly retrieve 

% it will learn how to match, now what is interesting is if we apply it in 

% Now, we note that 

% In order to learn a model that learns how to match for when X_q and X_k, , the attention forces it to learn but without overfitting, we early stop our model when the loss function hits a plateau. 

% Now, because  the key has exactly the information that the query is missing and our REBAR model is a map of the key to the output reconstruction, we should be able achieve perfect reconstruction when the model learns how to attend to the matching region in the key. This is illustrated in Fig. \ref{fig:validationtswithattn}a).
% \amnote{this is saying that if the key and query are the same, then they'll the same label and thus we want good reconstruction.}

In the \textit{contrastive learning stage}, we would like to identify whether an anchor time-series  $\textbf{X}_{anchor}$ and a candidate time-series $\textbf{X}_{cand}$, should be a positive or negative pair. Thus, we
\begin{align*}
    \textrm{Evaluate\ \ } d(\textbf{X}_{anchor}, {\textbf{X}}_{cand})\textrm{\ \ with\ \ } \textbf{X}_{anchor}  \neq \textbf{X}_{cand}
\end{align*}
% \begin{align*}
%     \textrm{Evaluate\ \ } \Vert\textrm{REBAR}(\bar{\textbf{X}}_{anchor}, {\textbf{X}}_{cand})-\textbf{X}_{anchor}\Vert_2^2 \textrm{\ \ with\ \ } \textbf{X}_{anchor}  \neq \textbf{X}_{cand}
% \end{align*}
With our trained REBAR cross-attention, the model will attempt to reconstruct $\bar{\textbf{X}}_{anchor}$ from $\textbf{X}_{cand}$, and we can use the reconstruction error as a quasi-distance between the two time series to form positive and negative pairs.

% %  \textrm{REBAR}(\bar{\textbf{X}}_1, {\textbf{X}}_2) \textrm{ and evaluate }
% REBAR's learned retrieval function, $p(\textbf{x}_k | \bar{\textbf{x}}_q)$, will search for the $\textbf{x}_k$ with the 
% to evaluate the similarity between
% best fit for our $\bar{\textbf{x}}_q$ and attempt to use this $\textbf{x}_k$ for reconstruction with $f_v(\textbf{x}_k)$ .
% The model will attempt to retrieve the matching region, but because the key and query are different, cannot find it, and instead will retrieve the one that matches the best and attempt to use that for reconstruction. 
% key and queries being different, and how the model will attempt to retrieve the matching region, even though it doesnt exist.
%to evaluate similarities between $\textbf{X}_q$ and $\textbf{X}_k$. 


% With our learned $p(\textbf{x}_k | \bar{\textbf{x}}_q)$ retrieval function, the model will search for the $\textbf{x}_{cand}$ with the best fit for our $\bar{\textbf{x}}_{anchor}$ and attempt to use this $\textbf{x}_{cand}$ for reconstruction with $f_v(\textbf{x}_{cand})$ . This is illustrated in Fig. \ref{fig:validationtswithattn}b) and c).

% \amnote{Now that we have a model that learns to retrieve, can appply on keys/queries not necessarily the same.}
% freeze $\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)$ and apply our model on examples in which $\textbf{X}_q \neq \textbf{X}_k$. 


We hypothesize that if we can retrieve information from one subsequence to successfully reconstruct the missing gaps in a different subsequence, then the two subsequences may share similar downstream labels. Then, this pair should be considered to be positive.  We investigate this hypothesis and harness this insight with our REtrieval-BAsed Reconstruction (REBAR) method. In REBAR, a cross-attention model retrieves information from one subsequence to reconstruct another. The ensuing reconstruction error is a metric to evaluate the similarity between the two, allowing us to identify positive and negative pairs to train our contrastive learning model to learn a class discriminative representation space. Note that we will interchangeably use "REBAR" to refer to the overall REBAR contrastive learning approach, the REBAR cross-attention module, and the REBAR metric, with the specific meaning being evident from the context. Our major contributions in this work are:

We seek to address this by exploiting how time-series can be understood as a sequence of subsequences. This is especially true for biophysical health signals: an active accelerometer sensor attached to a user outputs a single "complete" time-series over the course of a day. However, throughout the day, the user engages in different activities, such as walking and sitting, and each activity label generates a different temporal pattern within a subsequence. The time-series is composed of subsequences that are each an instantiation of a specific signal class. If we can capture the differences in the generative process among differing subsequences, then we can also capture information on whether they share the same class label or not.  

A key question for time-series contrastive learning is thus how to identify meaningful positive and negative pairs. We hypothesize that if one time-series is useful for reconstructing another, then they should form positive examples because they have mutual reconstruction information, perhaps through similar temporal structures or patterns. Our novel method, REBAR (REtrieval-BAsed Reconstruction), harnesses this insight and effectively establishes its suitability as a proxy for mutual class membership. We design our REBAR model with a convolutional cross-attention architecture that learns to retrieve temporal structures between differing time-series to effectively evaluate how one time-series can be used to reconstruct another. Then, once trained, REBAR simply serves as a positive/negative-labeler for the contrastive learning encoder, and thus is contrastive-learning-model agnostic and compatible with various encoder architectures. With the encoder as a control, we compare REBAR to other contrastive learning approaches and demonstrate REBAR's capability to achieve state-of-the-art results within a contrastive learning framework in downstream classification tasks across diverse data types.



\cut{
Self-supervised learning uses underlying structures found within data to learn rich and generalizable representations without labels, thus enabling fine-tuning on various downstream tasks. This reduces the need for large labeled datasets and has led to breakthroughs in computer vision with architectures such as SimCLR \citep{chen2020simclr}, SimSiam \citep{chen2021simsiam}, Masked Autoencoder \citep{he2022mae} and the natural language processing domain with architectures such as BERT \citep{devlin2018bert}. Self-supervised learning is an attractive approach for analyzing time series data, as it is increasingly feasible to capture a large volume of data with the advancement of sensor technologies, but the cost of data labeling remains high. For example, in mHealth applications \citep{Rehg2017mhealth} acquiring labels requires burdening participants by asking for annotations in real-time, while in medical applications such as ECG, annotation is costly due to the need for specialized medical expertise.

%jim's original -->> Self-supervised learning is an attractive approach for analyzing time series data, as it is increasingly feasible to capture a large volume of data, but the cost of data labeling remains high. For example, in mHealth applications \citep{Rehg2017mhealth} acquiring labels requires burdening participants by asking for annotations in real-time, while in medical applications such as ECG, annotation of traces is costly due to the need for specialized medical expertise.

%%It is particularly beneficial for sensor time series where high-frequency sensors can autonomously collect large volumes of unlabeled data, or in medical time series where annotation is costly due to the need for medical expertise. However, noisy time-series data presents unique challenges due to the low information content at each time point, similar to an individual pixel in an image, while also needing to capture long-range, complex temporal dependencies akin to word interactions within a paragraph.

% \textcolor{red}{not convincing as you just said these challenges are similar to other settings, then how are they unique?}

Contrastive learning is a successful self-supervised learning technique which is based on constructing positive and negative observation pairs and learning an embedding that preserves the similarity structure. In order to yield representations that are useful for downstream tasks, the process for generating positive and negative pairs must capture important structural properties of the data. In the computer vision applications that have driven contrastive learning, similarities can be easily obtained via the well-known invariances in the imaging process. Augmentations such as flipping, rotating, random cropping, and color jittering can be used to generate novel example images containing the same semantics as a source image. Representations that encode this similarity structure have been shown to be useful for downstream tasks such as image classification. Unfortunately, general time series signals don't possess a large and rich set of such invariances. Random cropping, which addresses translation or shift invariance, is widely-used, but other augmentations such as shuffling/permutations, magnitude scaling, or filtering can destroy the signal semantics. In ECG time series, for example, permuting samples destroys the temporal structure of the PQRS complex, while magnitude scaling changes the clinical meaning of the waveform. The existing literature does not paint a clear picture, for example methods such as TF-C \citep{zhang2022tfc} incorporate jittering and scaling, while TS2Vec \citep{yue2022ts2vec} finds that these augmentations reduce performance.

In this paper we explore a different approach to time series contrastive learning which is not based on exploiting invariances. Our approach is derived from a conceptual model for time series generation. In our model, a time series consists of a sequence of subsequences, where each subsequence is an instantiation of a temporal pattern from a certain signal class. In activity recognition, for example, a subject performs a set of activities in sequence, e.g. eating, walking, and then typing. These labelled activity subsequences are interspersed with intervals in which the participant's movements have no clear meaning. This conceptual model covers many of the time series data produced in mHealth applications, including accelerometry, ECG, and PPG waveforms. In classical supervised approaches, the subsequeces would be segmented, labeled, and used to train a model that could then detect the occurrence of each type of subsequence. In contrastive learning we assume we have access to the recorded time series data, without having any subsequence labels. Our approach is to sample subsequences within the time series and design a similarity function to quantify the similarity between subsequences. Subsequences that are similar would become positive examples for the purpose of learning an embedding via contrastive loss. Our key idea is to use reconstruction accuracy between two subsequences as the similarity function, where samples from one subsequence are used in a deep learning architecture to reconstruct the second subsequence. The intuition is that the more accurately one subsequence can be reconstructed from another one, the more likely it is that they share the same class label.

%%. It involves creating positive and negative observation pairs such that when positive pairs are drawn together and negative pairs apart in embedding space, the embedding captures semantic relationships in the data. In computer vision, where most contrastive learning work originates, constructing positive pairs is straightforward. Augmentations for images are designed for well-understood invariances like flipping and rotating, so that when used to form positive pairs, both the original image and its augmented counterpart maintain their semantic meaning. However, in time-series, augmentations in time-series are much trickier, as many risk changing the signal's semantic meaning (e.g. scaling ECG data may change the diagnosis) or destroy the temporal dependencies present (e.g. shuffling). Many of the augmentations used are often conflicting across different methods: TS2Vec \citep{yue2022ts2vec} explicitly found that jittering and scaling augmentations led to performance drops, but TF-C \citep{zhang2022tfc} then opts to use specifically include them.
% TS2Vec \citep{yue2022ts2vec} is a time-series contrastive learning method and uses only two augmentations, cropping and masking, and found that additional jittering/scaling augmentations led to performance drops. However, TF-C \citep{zhang2022tfc} opts to use jittering and scaling but requires additional frequency-based augmentations to achieve strong performance. TNC \citep{tonekaboni2021tnc} is one of the few non-augmentation-based approaches but suffers from slow run-time (250x slower than TS2Vec \citep{yue2022ts2vec}) and relies on a hyperparameter to estimate whether non-neighboring subsequences are truly negative.\textcolor{red}{you may want to just mention these papers without this much detail, and then add this level of detail and a bit more to the related work.}


% TS2Vec \citep{yue2022ts2vec} is a time-series contrastive learning method and uses only two augmentations, cropping and masking, and found that additional jittering/scaling augmentations led to performance drops. However, TF-C \citep{zhang2022tfc} opts to use jittering and scaling but requires additional frequency-based augmentations to achieve strong performance. TNC \citep{tonekaboni2021tnc} is one of the few non-augmentation-based approaches but suffers from slow run-time (250x slower than TS2Vec \citep{yue2022ts2vec}) and relies on a hyperparameter to estimate whether non-neighboring subsequences are truly negative.\textcolor{red}{you may want to just mention these papers without this much detail, and then add this level of detail and a bit more to the related work.}

% naively assumes stationarity is useful. 

In this paper we present a novel approach to self-supervised representation learning which leverages signal reconstruction as a similarity measure for matching portions of a time series within a single time series recording. Our approach leverages a basic property of how time series data is typically collected: Time series records are obtained within a specific context (e.g. a certain participant wearing a smart watch on their wrist), with durations ranging from hours to days. A single recording will contain many semantically-distinct segments, as in human activity recognition where a participant might ride a bike, dismount, lock the bike, and then start walking. If the samples corresponding to these different events were labelled, classic supervised learning methods could be applied. The question we address is how to identify segments which are more likely to belong to the same semantic class in the absence of labels. Our key idea is that if one portion of a time series is useful in reconstructing another portion, then those segments are more likely to have similar class labels and therefore should form positive examples.


A key question for time-series contrastive learning is thus how to identify meaningful positive and negative pairs. We hypothesize that if one time-series is useful for reconstructing another, then they should form positive examples because they have mutual reconstruction information, perhaps through similar temporal shapes or patterns. Our novel method, REBAR (REtrieval-BAsed Reconstruction), harnesses this insight and effectively establishes its suitability as a proxy for mutual class membership. We design our REBAR model with a convolutional cross-attention architecture that learns to retrieve temporal structures between differing time-series to effectively evaluate how one time-series can be used to reconstruct another. Then, once trained, REBAR simply serves as a positive/negative-labeler for the contrastive learning encoder, and thus is contrastive-learning-model agnostic and compatible with various encoder architectures. With the encoder as a control, we compare REBAR to other contrastive learning approaches and demonstrate REBAR's capability to achieve state-of-the-art results within a contrastive learning framework in downstream classification tasks across diverse data types.


% We demonstrate that when integrated into a contrastive learning framework, we showcase REBAR's capability to achieve state-of-the-art results in downstream classification tasks across a range of time-series datasets with diverse data types.


% , even before its utilization for contrastive learning
% say its encoder or model agnostic at some point.
To the best of our knowledge, our idea of using retrieval-reconstruction as a metric for contrastive learning is completely novel, even across other domains besides time-series. \emph{Therefore, our major contributions are:} 
1) We introduce a novel method of identifying positives and negatives for time-series contrastive learning with REtrieval-BAsed Reconstruction (REBAR). Our REBAR architecture leverages a convolutional cross-attention architecture in a novel way to do between-time-series retrieval and reconstruction. 2) To justify this approach and as a prequisite to contrastive learning, we demonstrate that the REBAR metric is a good proxy for mutual class membership between the two time-series 3) We benchmark our results against time-series datasets and show that our REBAR contrastive learning approach achieves state-of-the-art performance on learning an embedding space for three different sensor domains.

We first outline related work with other self-supervised learning works and retrieval-based methods in Sec \ref{sec:relatedwork}. Then we explain our REBAR architecture and application in contrastive learning in Sec \ref{sec:method}. Finally, we present our experiments and results in Sec \ref{sec:experiments} and discuss avenues for future work. 
}




In the contrastive learning stage, we can use a frozen REBAR cross-attention to identify  whether an anchor and a candidate subsequence should form a positive or negative pair.
% \begin{align*}
%     \textrm{Evaluate\ \ } \Vert\textrm{REBAR}(\bar{\textbf{X}}_{anchor}, {\textbf{X}}_{cand})-\textbf{X}_{anchor}\Vert_2^2 \textrm{\ \ with\ \ } \textbf{X}_{anchor}  \neq \textbf{X}_{cand}
% \end{align*}
With our trained $\textrm{REBAR}(\bar{\textbf{X}}_q, {\textbf{X}}_k)$, the model will attempt to reconstruct $\bar{\textbf{X}}_{anchor}$ from $\textbf{X}_{cand}$, and we can use the reconstruction error within a contrastive learning framework. Given a time-series, we uniformly at random sample an anchor subsequence, $\textbf{X}_{anchor}$, and $n$ candidate subsequences,  $\textbf{X}_{cand}$, that make up the set $\mathcal{S}_{cand}$. We can then use REBAR to label our candidates:
% We then evaluate each of these $n$ candidate time-series as the key input with the REBAR model with $\bar{\textbf{X}}_{anchor}$ as the query. 

% With our trained REBAR cross-attention, the model will attempt to reconstruct $\bar{\textbf{X}}_{anchor}$ from $\textbf{X}_{cand}$, and we can use the reconstruction error to predict whether the two subsequences share a mutual class and use this to label a pair as being either positive or negative. \amnote{how? I would `expect' there to be a threshold but you mentioned something else. normalize mse into probability then sample from them, sample from them, lay it out and then point at future works}

The linear layer following the cross-attention module is used to project the subsequence from the embedding space back to its original dimension. 

This allows for the emphasis to be on learning a good retrieval function, $p(\textbf{x}_k | \bar{\textbf{x}}_q)$ rather than learning a complicated layers after the cross-attention, which may learn to reconstruct the original signal 

Therefore, it is important to note that \textit{the query subsequence is not directly used for this reconstruction, it is only used to identify regions in the key subsequence to retrieve with $p(\textbf{x}_k | \bar{\textbf{x}}_q)$.} By using cross-attention to model our query reconstruction, we cannot ``cheat'' by borrowing information from the query itself for reconstruction. The reconstruction information only flows from the retrieved regions of the key subsequence with $f_v(\textbf{x}_{k})$ and 

In our framework, we define a time-series as being a composition of a series of subsequences, each of which has a class label. This conceptualization describes many real-world physiological signals. For example, a participant wearing an accelerometer generates a time-series over the course of a day which consists of a series of subsequences of different activities such as sitting and walking. Each subsequence is an instantiation of a specific class of activities, and subsequences with the same class label are likely to have similar temporal patterns. Therefore, two subsequences with similar temporal patterns would be a good candidate to form a positive pair.


In our framework, we define a time-series as being a composition of a series of subsequences, each of which has a class label. This conceptualization describes many real-world physiological signals. For example, a participant wearing an accelerometer generates a time-series over the course of a day which consists of a series of subsequences of different activities such as sitting and walking. Each subsequence is an instantiation of a specific class of activities, and subsequences with the same class label are likely to have similar temporal patterns. Therefore, two subsequences with similar temporal patterns would be a good candidate to form a positive pair.



for shapelet 
The idea of utilizing temporal shape in time-series tasks has been widely studied,




The identify of shape-based learning for time-series classification is well-studied, particularly in the context of template, shape

The importance of shapes in identifying 


This idea of  using temporal patterns to study stuff is not new, we have seen it before in a lot of Eamon Keoughs work with matrix profiles and identifications

shapelet approaches

However, these works fail to do  few works manage to use it as a guide 


We propose to measure the similarity between two subsequences by using one subsequence to reconstruct the other one, and taking the reconstruction error as a quasi-distance metric. 

In this work, we introduce a novel approach to identifying positive and negative pairs for contrastive time-series learning through a "motif-based" retrieval and reconstruction method. In our framework, we define a time-series as being a composition of a series of subsequences, each of which has a class label. This conceptualization describes many real-world physiological signals. For example, a participant wearing an accelerometer generates a time-series over the course of a day, which consists of a series of subsequences. Each subsequence has individual activity labels (e.g. sitting and walking) and contains brief temporal shapes or "motifs" that are an instantiation of that specific activity class. Therefore, two subsequences with similar temporal patterns would be a good candidate to form a positive pair.


The idea that specific class-discriminative "motifs" within a sequence has been widely-studied and validated in time-series data mining \citep{yeh2018time, yeh2016matrix, alaee2021time}.

The idea that specific class-discriminative "motifs" within a sequence has been widely-studied and validated in time-series data mining \citep{yeh2018time, yeh2016matrix, alaee2021time}.
class-discriminative "motifs" are definitley present within sequences and have been studied extensively in the time-series data mining literature. 

The idea of identifying specific class-discriminative "motifs" within the sequence has been widely-studied for time-series data mining \citep{yeh2018time, yeh2016matrix, alaee2021time}, but there are very few works that exploit this idea for unsupervised deep-learning. 


This idea of identifying class-discriminative motifs and exploiting temporal shape information for classification has been widely-studied within time-series data mining \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}, and so we argue that two subsequences with similar temporal patterns would be a good candidate to form a positive pair. 

. This will then lead to similar reconstruction performance, thereby reducing the model's discriminative capability. Thus, we would like to use a contiguous mask during training, which masks out larger, potential class-discriminative motifs. For example, by masking out an entire heartbeat, the model will have different reconstruction performance when 


Reconstructing a normal signal from one with misshapen heartbeats will have a higher error than reconstructing from another normal signal. 




entire temporal shapes.  

Fig. \ref{fig:extendedortrain}a) shows that the attention weights learned with a contiguous mask are sparse and fit exactly onto the region in the key corresponding to the masked region in the query. If we use an intermittent mask, the model matches many different temporal shapes throughout the key, which is shown in Fig \ref{fig:extendedortrain}b)'s dispersed attention distribution. This is an issue because the model cannot retrieve class-specific motifs, choosing instead to match with minor


\responsehide{\amnote{I wouldn't say minor. Really there are several things in a time series: trend, cycle, periodicity, noise. What is it matching among these? Are you sure it is trend?}, i am not sure, its kind of a bastardization of the word "trend". lets discuss}

, transient trends. The use of a contiguous mask encourages the model to learn to attend to specific temporal shapes in the key.

A common paradigm in working with time-series data collected over a long period of time (e.g. hours or days) is to partition it into shorter contiguous subsequences (e.g. at the level of seconds or minutes, respectively) for labeling and classification. Throughout this paper, we shall refer to the partitions of a longer time-series signal as subsequences. Sampling-based methods attempt to capture the evolving dynamics present in the time-series by sampling subsequences to construct positive pairs. 

Before its use in contrastive learning, REBAR's effectiveness in identifying pos/neg examples can be evaluated in a validation experiment. Given an anchor subsequence, we sample a candidate subsequence from each class, and the anchor subsequence is predicted to be the class of the candidate with the lowest REBAR error with a masked-out anchor. The mean of the bootstrapped accuracies is shown.

Given a query, a retrieval function searches for the most useful information within a database that can be used for some downstream task. In our setting, this query is a query subsequence, and the database is a different key subsequence. ,

If the model is only trained to reconstruct transient motifs, like a short upward slope, both healthy and unhealthy signals will exhibit this motif, so both signals will be able to reconstruct a short upwards slope similarity. This means that we cannot use differences in reconstruction performance to indicate class differences. Fig. \ref{fig:extendedortrain}b) shows that training with the transient mask results in a dispersed attention distribution, which means that the model is retrieving minor, non-unique motifs. Therefore, we use contiguous mask during training, which masks out larger, potential class-discriminative motifs. When reconstructing an entire healthy heartbeat, the model will tend to have better performance when retrieving a matching motif from a healthy signal versus retrieving the motif from an unhealthy one. Fig. \ref{fig:extendedortrain}a) shows that the attention weights learned with a contiguous mask are sparse and fit exactly onto the region in the key corresponding to the masked region in the query, and thus the model has learned to retrieve specific motifs. 


This loss learns to pull the anchor and the subsequence that is most likely to be of the same class as the anchor, according to REBAR, together in the embedding space, while pushing the anchor and the subsequences with higher REBAR error apart. This allows us to capture the differences in states between subsequences in our embedding space. Our full REBAR approach is visualized in Fig \ref{fig:rebarfull}.

This allows us to capture the evolving dynamics
found within one subject’s signal over time
 The candidate with the lowest REBAR error is labeled as the \textit{positive}, $\textbf{X}_{pos}$, because as we shown in the prior sections, REBAR is an unsupervised predictor for mutual class membership. All of the other candidates are  \textit{within-subject negatives}, in the $\mathcal{S}_{within-neg}$ because their REBAR error is not as good as the positive example.




During application, we use an intermittent mask. Fig. \ref{fig:extendedortrain} shows that the model trained with a contiguous mask still maintains a sparse attention when applied with an intermittent mask, and so, the query is still reconstructed based on specific motifs from the key. Because the masked points are dispersed in an intermittent mask, we can evaluate motif-similarity via REBAR throughout the query for a better comparison with the key. This masking idea is further explained and empirically validated in Appendix \ref{sec:maskingval}.



We describe our REBAR cross-attention model with a retrieval formulation below with the scaling factor, biases, norms, and aggregation linear layer omitted for brevity:
% Cross-attention is an attractive method for modeling this paradigm as the attention weights can be interpreted as a retrieval function. Cross-attention learns a weighted average of a transformation of the key time-series, and the weights are a learned similarity between the query and keys. We describe it in our reconstruction setting with its expected value formulation below \citep{tsai2019transformerkernel}:
% and thus allows us to 
% we pool at loss function step
% is a weighted , as it allows us 
% with a strong inductive bias \textcolor{red}{why does it have strong inductive bias? do you have any evidence of that?}for this problem, and is described below with it's expected value formulation \textcolor{red}{in one brief sentence, describe the intuition for cross attention: weighted average of values, conditional on keys, describe how it's doing smoothing}:
\begin{align}
    \textrm{REBAR}(\bar{\textbf{x}}_q ; {\textbf{X}_k}) 
    & = \sum_{\textbf{x}_k \in {\textbf{X}_k}} \frac{\exp(\langle f_q( \bar{\textbf{x}}_{q} ), f_k( \textbf{x}_{k}) \rangle )} {\sum_{\textbf{x}_k' \in {\textbf{X}_k'}} {\exp( \langle f_q( \bar{\textbf{x}}_{q} ), f_k( \textbf{x}_{k'}) \rangle )}}  f_v( \textbf{x}_{k}) \label{eq:rebarissoftmax} \\
    % \textbf{x}_{k} \textbf{W}_v
    % &= \sum_{\textbf{x}_k \in S_{\textbf{X}_k}} \frac{k (\textbf{x}_q, \textbf{x}_k)}{\sum_{x_k' \in S_{\textbf{X}_k'}} k (\textbf{x}_q, \textbf{x}_k')} v(\textbf{x}_k) \\
    &= \sum_{\textbf{x}_k  \in  {\textbf{X}_k}}  p(\textbf{x}_k | \bar{\textbf{x}}_q) f_v( \textbf{x}_{k}) \label{eq:rebarisretrieval}
    % &= \mathbb{E}_{p(\textbf{x}_k|\bar{\textbf{x}}_q)}[f_v( \textbf{x}_{k})]
\end{align}
% with the full cross-attention network, $\textrm{g}(\textbf{x}_q ; {\textbf{X}_k}) $, described as 
% \begin{align*}
%     \textrm{g}(\textbf{x}_q ; {\textbf{X}_k}) 
%     & = \textrm{CrossAttn}(\textbf{x}_q ; {\textbf{X}_k}) W_L
% \end{align*}



In a vanilla cross-attention, each of the $f$ embedding functions could be understood as a convolution with a kernel size of 1:
$f_q( \bar{\textbf{x}}_{q} ) =  \bar{\textbf{x}}_{q} \textbf{W}_q $, $f_k( \textbf{x}_{k} ) =  \textbf{x}_{k} \textbf{W}_k $, $f_v( \textbf{x}_{k} ) =  \textbf{x}_{k} \textbf{W}_v $,  with $\textbf{W}_{\{q/k/v\}} \in \mathbb{R}^{D_x \times D}$. 




which identifies regions in the key subsequence useful for the reconstruction downstream task based on the $\langle f_q( \bar{\textbf{x}}_{q} ), f_k( \textbf{x}_{k}) \rangle $ calculation found in Eq. \ref{eq:rebarissoftmax}. 



 in Eq. \ref{eq:rebarisretrieval} is the retrieval function, which identifies regions in the key subsequence useful for the reconstruction downstream task based on the $\langle f_q( \bar{\textbf{x}}_{q} ), f_k( \textbf{x}_{k}) \rangle $ calculation found in Eq. \ref{eq:rebarissoftmax}. 

$p(\textbf{x}_k | \bar{\textbf{x}}_q)$ in Eq. \ref{eq:rebarisretrieval} is the retrieval function, which identifies regions in the key subsequence useful for the reconstruction downstream task based on the $\langle f_q( \bar{\textbf{x}}_{q} ), f_k( \textbf{x}_{k}) \rangle $ calculation found in Eq. \ref{eq:rebarissoftmax}. 



However, vanilla $f_{k/q}$ in the original transformer paper \citep{vaswani2017attnisallyouneedtransformer} is calculated with only a single time-point, which holds limited information about its semantic content. We would instead like our retrieval-function to retrieve motifs for reconstruction, so that reconstruction performance is directly dependent on motif-similarity. Therefore, we utilize a dilated convolution for $f_{k/q/v}$ to capture information from the wider surrounding temporal neighborhood \citep{xu2022pulseimpute}. The $f_{k/q}$ dilated convs allow for motif-similarity comparison to identify regions in $\textbf{X}_{k}$ for retrieval, and then the $f_{v}$ consolidates information from that region for reconstruction. The reversible instance norm (RevIN) \citep{kim2021revin} normalizes the data at input, before reversing it at the output for reconstruction. We opt to not use positional encoding so that the retrieval function focuses on learning a good motif comparison function, rather than considering specific positions of the motifs. The full block diagram is shown in \ref{fig:rebarfull}a), and further model details can be found in Appendix \ref{sec:morerebarcrossdetail}.


\subsection{Intuition} \label{sec:method}
If two subsequences are instantiations of the same class, then they likely to share similar temporal shapes and patterns. This is corroborated by the extensive time-series motif literature, which seeks to identify class-discriminative motifs \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}. Our approach builds upon this with two key ideas: 


\textbf{Key Idea (1): We can capture motif-similarity with retrieval-based reconstruction.} Our REBAR model reconstructs $\bar{\textbf{X}}_{anchor}$ by retrieving motifs in ${\textbf{X}}_{cand}$ that match the not-masked context.



% Then if we label subsequences close together as positive pairs and those further apart as negative, then we can learn a class-discriminative space.
\textbf{Key Idea (2): The ensuing retrieval-based reconstruction error captures semantic relationships, useful for guiding contrastive learning.} REBAR error serves as a quasi-distance metric between two sequences, shown below in Eq. \ref{eq:rebardistance}. When pairs with lower error are grouped together and those with higher error should be pushed apart in a contrastive learning approach, the ensuing embedding space would be useful for downstream tasks.

\begin{align}
    d(\textbf{X}_{anchor},\textbf{X}_{cand})&=\Vert\textrm{REBAR}(\bar{\textbf{X}}_{anchor}, {\textbf{X}}_{cand})-\textbf{X}_{anchor}\Vert_2^2 \label{eq:rebardistance}
\end{align}


While not a valid distance metric (violating symmetry and the triangle inequality), positivity is likely to hold, as we would need perfect reconstruction for it not to, and we can train $\textrm{REBAR}$ to approximate the distance to itself is (approximately) zero. We hypothesize that if $d(\textbf{X}_{anchor},\textbf{X}_{cand})$ is small, then it predicts if $y(\textbf{X}_{anchor} ) = y(\textbf{X}_{cand})$, allowing us to identify positive and negative pairs for contrastive learning, which we do confirm in our validation experiments in Sec. \ref{sec:rebarunderstand}.


In our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, and the REBAR metric. The specific meaning will be evident from the context.} approach, we propose to measure the similarity between two subsequences by retrieving motifs in one subsequence conditioned on the unmasked motifs in the other, to reconstruct the other subsequence's masked-out points. The ensuing reconstruction error is a quasi-distance measure that captures motif similarity. Pairs with a closer distance can then form positive examples in contrastive learning. We illustrate this idea in Fig. \ref{fig:intuition}. Because the pair is likely to share the same class label (which we validate prior to  contrastive learning), then the resulting learned embedding space is likely to be class-discriminative. 


Therefore, if two subsequences are semantically related, then they are likely to share similar motifs. 


% Additionally, framing our work in the context of time-series signals that model an changing state over time, allow us to leverage and benchmark sampling-based contrastive learning approaches, such as TNC \citep{tonekaboni2021tnc}, in which a positive pairs are sampled directly from the original long time-series.

% Prior work has been done on identifying such 



% This idea of identifying class-discriminative motifs and exploiting temporal shape information for classification has been widely-studied within time-series data mining \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}, and so we argue that two subsequences with similar temporal patterns would be a good candidate to form a positive pair.

%It follows that if we have a way to quantify the extent to which two subsequnces have a similar temporal pattern, this could be used to identify subsequences that share the same class label.
%the similarity between two subsequences, this could be used to identify subsequences that share the same label.

% It follows that 
%%We seek to address this by exploiting how time-series can be understood as a sequence of subsequences. This is especially true for biophysical health signals: an active accelerometer sensor attached to a user outputs a single "complete" time-series over the course of a day. However, throughout the day, the user engages in different activities, such as walking and sitting, and each activity label generates a different temporal pattern within a subsequence. The time-series is composed of subsequences that are each an instantiation of a specific signal class. If we can capture the differences in the generative process among differing subsequences, then we can also capture information on whether they share the same class label or not.  
% reconstruct the signal in a way that preserves class discriminative information
% REBAR error is a proxy for mutual class membership, 
% the class-discriminative features
% % While missing data has been widely studied in statistics~\citep{Little2020missingdata} and machine learning \citep{fang2020timeseriesmlimp}, very few works have systematically addressed missing pulsative data and even fewer in an mHealth field context, despite this setting's importance and interesting nature. We define a set of criteria  necessary to comprehensively study this setting found in the rows of Tbl. \ref{tbl:necessarycomp} and find that our PulseImpute Challenge is the only work to address all of them.
% The value of temporal shape information has been widely studied and validated for time-series data mining \citep{yeh2018time}, and much of the prior work has focused on isolating and identifying specific short class-discriminative "motifs" within the sequence \citep{yeh2016matrix}. 
% We design our REtrieval-BAsed Reconstruction (REBAR)  around a convolutional cross-attention model
% however, these works are primarily focused upon learning or identifying templates 
% and here we seek to exploit this idea within a unsupervised deep-learning context. 
% The idea of identifying specific class-discriminative "motifs" within the sequence has been widely-studied for time-series data mining \citep{yeh2018time, yeh2016matrix}, but there are very few works that exploit this idea forin the unsupervised deep-learning space. In REtrieval-BAsed Reconstruction (REBAR)\footnote{Note that we interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention module, and the REBAR metric. The specific meaning will be evident from the context.}, we propose to measure the similarity between two subsequences by retrieving motifs from one subsequences to reconstruct the missing motifs in the other with a convolutional cross-attention mechanism. Then, we are able show that the ensuing reconstruction error is a good predictor for mutual class membership. This validates our approach to label pairs with low error as positive in a contrastive learning approach, encouraging for the learned embedding space to be class-discriminative. Our learned embedding space achieves SOTA classification results with a linear probe and in clusterability evaluations. Our major contributions in this work are:
% We propose to measure the similarity between two subsequences by using one subsequence to reconstruct the other one, and taking the reconstruction error as a similarity measure. Pairs with low reconstruction error can then form positive examples in contrastive learning. Because the pair is likely to share the same class label, the resulting learned embedding space is likely to be class-discriminative.

% by retrieving motifs from one subsequence to reconstruct the missing motifs in the other with a convolutional cross-attention mechanism. Then, we are able show that the ensuing reconstruction error is a good predictor for mutual class membership. This validates our approach to label pairs with low error as positive in a contrastive learning approach, encouraging for the learned embedding space to be class-discriminative. Our learned embedding space achieves SOTA classification results with a linear probe and in clusterability evaluations. 
%%We hypothesize that if one time-series is useful for reconstructing another, then they should form positive examples because they share reconstruction information, perhaps through similar temporal structures or patterns. 
% 1) We introduce a novel method of identifying positives and negatives for time-series contrastive learning with our REBAR metric, calculated from a convolutional cross-attention architecture that does between-sequence retrieval and reconstruction. 2) To justify this approach and as a pretext to contrastive learning, we demonstrate that the REBAR metric is a good proxy for mutual class membership between the two time-series 3) We benchmark our results against time-series datasets and show that our REBAR contrastive learning approach achieves state-of-the-art performance on learning an embedding space for three distinctive sensor domains.

Now, we introduce our REBAR approach. Following our \textbf{Key Idea (1)}, our REBAR cross-attention architecture reconstructs $\bar{\textbf{X}}_{anchor}$ by retrieving motifs in ${\textbf{X}}_{cand}$ that match the not-masked context, and this is described in Sec. \ref{sec:rebararch}. Then, REBAR error serves as a quasi-distance metric between two sequences, shown below in Eq. \ref{eq:rebardistance}. 

\begin{align}
    d(\textbf{X}_{anchor},\textbf{X}_{cand})&=\Vert\textrm{REBAR}(\bar{\textbf{X}}_{anchor}, {\textbf{X}}_{cand})-\textbf{X}_{anchor}\Vert_2^2 \label{eq:rebardistance}
\end{align}
Then, with \textit{Key Idea (2)}, Sec. \ref{sec:rebarapply}, when pairs with lower error are grouped together and those with higher error should be pushed apart in a contrastive learning approach, the ensuing embedding space would be useful for downstream tasks.




Following \textit{Key Idea (1)},  describes our cross-attention architecture for learns a retrieval-based reconstruction that captures motif-similarity.  explains how to apply the model for subsequence comparison in a contrastive learning framework. 




While not a valid distance metric (violating symmetry and the triangle inequality), positivity is likely to hold, as we would need perfect reconstruction for it not to, and we can train $\textrm{REBAR}$ to approximate the distance to itself is (approximately) zero. We hypothesize that if $d(\textbf{X}_{anchor},\textbf{X}_{cand})$ is small, then it predicts if $y(\textbf{X}_{anchor} ) = y(\textbf{X}_{cand})$, allowing us to identify positive and negative pairs for contrastive learning, which we do confirm in our validation experiments in Sec. \ref{sec:rebarunderstand}.



when pairs with lower error are grouped together and those with higher error should be pushed apart the ensuing embedding space would be useful for downstream tasks.


explains how to apply the model for subsequence comparison in a contrastive learning framework. 




our REBAR approach. Following our \textbf{Key Idea (1)}, our REBAR cross-attention architecture reconstructs $\bar{\textbf{X}}_{anchor}$ by retrieving motifs in ${\textbf{X}}_{cand}$ that match the not-masked context, and this is described in Sec. \ref{sec:rebararch}. Then, REBAR error serves as a quasi-distance metric between two sequences, shown below in Eq. \ref{eq:rebardistance}. 






metric that 

Sec. \ref{sec:rebararch} describes our cross-attention module for learning the REBAR metric,






our REBAR approach. From \textbf{Key Idea (1)}, 



If two subsequences are instantiations of the same class, then they likely to share similar temporal shapes and patterns. This is corroborated by the extensive time-series motif literature, which seeks to identify class-discriminative motifs \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}. Our approach builds upon this with two key ideas: 


\textbf{Key Idea (1): We can capture motif-similarity with retrieval-based reconstruction.} Our REBAR model reconstructs $\bar{\textbf{X}}_{anchor}$ by retrieving motifs in ${\textbf{X}}_{cand}$ that match the not-masked context.



% Then if we label subsequences close together as positive pairs and those further apart as negative, then we can learn a class-discriminative space.
\textbf{Key Idea (2): The ensuing retrieval-based reconstruction error captures semantic relationships, useful for guiding contrastive learning.} 




Our approach utilizes retrieval-based reconstruction, REBAR, as a metric for contrastive learning, as it is a strong predictor for mutual class membership between subsequences, and the full REBAR contrastive learning approach is shown in Fig. \ref{fig:rebarfull}. 









% \subsection{Notation} \label{sec:notation}
% innovative idea that


% The embeddings of $\textbf{X}_{anchor}$ and $\textbf{X}_{pos}$ are pulled together and the embeddings of $\textbf{X}_{anchor}$ and $\textbf{X}_{neg}$ are pushed apart. 
% and will use this time-series and subsequence framing for the rest of our paper. Specifically, $\textbf{A} \in \mathbb{R}^{U \times D}$, is a time-series, where $U$ is length and $D$ is channel. $\textbf{X} \in \mathbb{R}^{T \times D}$ with $T \ll U$ is a segmented subsequence from $\textbf{A}$. The time-series $\textbf{A}$ has changing dynamic states (e.g. a PPG signal measuring fluctuating stress states) over time so that a given subsequence $\textbf{X}$ may have a specific classification label (e.g. stressed, not stressed). 



\subsection{Intuition} \label{sec:method}
If two subsequences are instantiations of the same class, then they likely to share similar temporal shapes and patterns. This is corroborated by the extensive time-series motif literature, which seeks to identify class-discriminative motifs \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}. Our approach builds upon this with two key ideas: 


\textbf{Key Idea (1): We can capture motif-similarity with retrieval-based reconstruction.} Our REBAR model reconstructs $\bar{\textbf{X}}_{anchor}$ by retrieving motifs in ${\textbf{X}}_{cand}$ that match the not-masked context.



% Then if we label subsequences close together as positive pairs and those further apart as negative, then we can learn a class-discriminative space.
\textbf{Key Idea (2): The ensuing retrieval-based reconstruction error captures semantic relationships, useful for guiding contrastive learning.} 


% , a characterization which describes many physiological signals
% \responsehide{\amnote{contiguous } you keep saying contiguous but im not sure you understand what im saying, lets discuss. the subsequences are not necessarily contiguous, especially when finding random positive and negatives}


% \amnote{Going forward, any further mentions of subsequences are implied to be contiguous}

% Retrieval-Enhanced Transformer \citep{borgeaud2022retro}, while having a similar naming scheme, does not use the transformer for retrieval, unlike our approach. Instead, they use a kNN method to retrieve the most relevant documents to the query sentence input. 
Following \textit{Key Idea (1)}, Sec. \ref{sec:rebararch} describes our cross-attention architecture for learns a retrieval-based reconstruction that captures motif-similarity. Then, REBAR error serves as a quasi-distance metric between two sequences, shown below in Eq. \ref{eq:rebardistance}. With \textit{Key Idea (2)}, Sec. \ref{sec:rebarapply} shows how to use the REBAR metric in a contrastive learning approach, to identify positive and negative pairs. 
\begin{enumerate}[leftmargin=*,noitemsep,nosep]
\item We introduce a novel method of identifying positives and negative pairs with our REBAR metric, calculated from a convolutional cross-attention architecture that does between-sequence retrieval and comparison of potential class-specific motifs.
\item To justify this approach and as a prerequisite to contrastive learning, we show that the REBAR metric predicts mutual class membership of two subsequences.
\item Our REBAR contrastive learning approach achieves SOTA performance against a representative suite of methods that each utilize a different method of creating pos/neg pairs, demonstrating REBAR's strength in identifying meaningful semantic relationships for contrastive learning.
\end{enumerate}




% \vspace{-1mm}
% \begin{itemize}[leftmargin=*,noitemsep,nosep,wide = 0pt]
% \item \textit{Key Idea (1): We can capture motif-similarity with retrieval-based reconstruction.} Our REBAR model reconstructs a partially-masked  anchor sequence by retrieving motifs in a candidate sequence that match the not-masked motifs in the anchor sequence. 
% \item \textit{Key Idea (2): The ensuing retrieval-based reconstruction error captures semantic relationships, useful for guiding contrastive learning.} We illustrate this intuition in Fig. \ref{fig:intuition}. REBAR error serves as a quasi-distance metric between two sequences, and pairs with a closer distance can then form positive examples in contrastive learning. Because the pair is likely to share the same class label, then the resulting learned embedding space is likely to be class-discriminative. 
% \end{itemize}



Therefore, we design REBAR such that the reconstruction is directly dependent

Retrieval-based reconstruction retrieves the most useful information in one subsequence to reconstruct another. 



forcing the model to reconstruct only based on 


how to effectively retrieve and compare motifs between subsequences rather than learning temporal dependencies within the query. 



shittily when shitty motifs are present in the key and reconstruct well 

shitty motifs when shitty motifs are present and retrieve good motifs 


. Therefore


Our objective is to learn a good retrieval function, $p(\textbf{x}_k | \bar{\textbf{x}}_q)$ that measures similarity of temporal structures between $\textbf{X}_q$ and ${\textbf{X}}_k$. As such, we intentionally utilize a simple approach. 

The retrieval function is the only place in which the query subsequence is used so we cannot borrow information from the query itself for reconstruction. 
The reconstruction information only flows from the retrieved regions of the key subsequence with $f_v(\textbf{x}_{k})$ forcing the model to learn how to effectively retrieve and compare motifs between subsequences rather than learning temporal dependencies within the query. 

 Specifically,  from the time-series $\textbf{A}^{(i)}$, we randomly segment out one anchor subsequence, $\textbf{X}_{anchor, 0}^{(i)}$ and $C$ candidate subsequence, $\textbf{X}_{cand, 0}^{(i)}, \cdots, \textbf{X}_{cand, C}^{(i)}$, from each of the $C$ classes, where the number after the comma designates the true class label. Then, the anchor subsequence's class is predicted to be the class of the candidate that provided the lowest REBAR error (i.e. $    \textrm{pred}(\textbf{X}_{anchor}^{(i)}) = \textrm{argmin}_{c} d({\textbf{X}}_{anchor, 0}^{(i)}, {\textbf{X}}_{cand, c}^{(i)})$)


Specifically,  from the time-series $\textbf{A}^{(i)}$, we randomly segment out one anchor subsequence, $\textbf{X}_{anchor, 0}^{(i)}$ and $C$ candidate subsequence, $\textbf{X}_{cand, 0}^{(i)}, \cdots, \textbf{X}_{cand, C}^{(i)}$, from each of the $C$ classes, where the number after the comma designates the true class label. Then, the anchor subsequence's class is predicted to be the class of the candidate that provided the lowest REBAR error (i.e. $    \textrm{pred}(\textbf{X}_{\textrm{anchor}}^{(i)}) = \textrm{argmin}_{c} d({\textbf{X}}_{anchor, 0}^{(i)}, {\textbf{X}}_{cand, c}^{(i)})$)


The above procedure is run, then repeated for a anchor of each class, then repeated each time-series to obtain an average of the class prediction accuracy. The results are show in the confusion matrices in Fig. \ref{fig:confusion} below. 

Additionally, Fig. \ref{fig:extendedortrain} visualizes the reconstruction of an anchor subsequence with different candidate subsequences along with its attention weights. Fig. \ref{fig:extendedortrain}b) and c) show that despite being trained with the key and the query being the same instance, REBAR model is still able to reconstruct the query when the key is different. The attention weights retrieve the most relevant information from the key, and the weights being sparse indicates that specific motifs are being retrieved and compared. 



The trained REBAR cross-attention can be used to attempt to reconstruct $\bar{\textbf{X}}_{\textrm{anchor}}$ from $\textbf{X}_{\textrm{cand}}$ in which $\textbf{X}_{\textrm{anchor}}  \neq \textbf{X}_{\textrm{cand}}$. Then, we can use the ensuing reconstruction error to label the candidates. 

From the $i$th time-series $\textbf{A}^{(i)}$, we uniformly random sample an anchor subsequence, $\textbf{X}_{\textrm{anchor}}^{(i)}$, and $n$ candidate subsequences, $\textbf{X}_{\textrm{cand}}^{(i)}$, which make up the set $\mathcal{S}_{\textrm{cand}}^{(i)}$. Then, we can label the candidates to be the positive, $\textbf{X}_{\textrm{pos}}^{(i)}$, or to be the within-time-series negative set $\mathcal{S}_{\textrm{within-neg}}^{(i)}$.
\begin{align}
    \textbf{X}_{\textrm{pos}}^{(i)} &=  \underset{{\textbf{X}}_{\textrm{cand}}^{(i)} \in \mathcal{S}_{\textrm{cand}}^{(i)}}{\textrm{argmin}}  d(\textbf{X}_{\textrm{anchor}}^{(i)}, {\textbf{X}}_{\textrm{cand}}^{(i)}) \nonumber \\ % \label{eq:pos}\\ % \underset{{\textbf{X}}_{\textrm{cand}} \in \mathcal{S}_{\textrm{cand}}}{\textrm{argmin}}  \Vert\textrm{REBAR}(\bar{\textbf{X}}_{\textrm{anchor}}, {\textbf{X}}_{\textrm{cand}})-\textbf{X}_{\textrm{anchor}}\Vert_2^2 \\
    \mathcal{S}_{\textrm{within-neg}}^{(i)} &= \mathcal{S}_{\textrm{cand}}^{(i)} \setminus \{\textbf{X}_{\textrm{pos}}^{(i)}\} \nonumber % \label{eq:neg}
\end{align}

while if we define $\mathcal{S}_{\textrm{neg}}^{(i)}\equiv$, then we have ...




The trained REBAR cross-attention can be used to attempt to reconstruct $\bar{\textbf{X}}_{\textrm{anchor}}$ from $\textbf{X}_{\textrm{cand}}$ in which $\textbf{X}_{\textrm{anchor}}  \neq \textbf{X}_{\textrm{cand}}$. Then, we can use the ensuing reconstruction error to label the candidates. 

From the $i$th time-series $\textbf{A}^{(i)}$, we uniformly random sample an anchor subsequence, $\textbf{X}_{\textrm{anchor}}^{(i)}$, and $n$ candidate subsequences, $\textbf{X}_{\textrm{cand}}^{(i)}$, which make up the set $\mathcal{S}_{\textrm{cand}}^{(i)}$. Then, we can label the candidates to be the positive, $\textbf{X}_{\textrm{pos}}^{(i)}$, or to be the within-time-series negative set $\mathcal{S}_{\textrm{within-neg}}^{(i)}$.
\begin{align}
    \textbf{X}_{\textrm{pos}}^{(i)} &=  \underset{{\textbf{X}}_{\textrm{cand}}^{(i)} \in \mathcal{S}_{\textrm{cand}}^{(i)}}{\textrm{argmin}}  d(\textbf{X}_{\textrm{anchor}}^{(i)}, {\textbf{X}}_{\textrm{cand}}^{(i)}) \nonumber \\ % \label{eq:pos}\\ % \underset{{\textbf{X}}_{\textrm{cand}} \in \mathcal{S}_{\textrm{cand}}}{\textrm{argmin}}  \Vert\textrm{REBAR}(\bar{\textbf{X}}_{\textrm{anchor}}, {\textbf{X}}_{\textrm{cand}})-\textbf{X}_{\textrm{anchor}}\Vert_2^2 \\
    \mathcal{S}_{\textrm{within-neg}}^{(i)} &= \mathcal{S}_{\textrm{cand}}^{(i)} \setminus \{\textbf{X}_{\textrm{pos}}^{(i)}\} \nonumber % \label{eq:neg}
\end{align}




The trained REBAR cross-attention can be used to attempt to reconstruct $\bar{\textbf{X}}_{\textrm{anchor}}$ from $\textbf{X}_{\textrm{cand}}$ in which $\textbf{X}_{\textrm{anchor}}  \neq \textbf{X}_{\textrm{cand}}$. As previously discussed, the subsequent reconstruction error acts as a proxy for mutual class membership due to the motif retrieval and reconstruction properties, and it is validated empirically in Sec. \ref{sec:rebarunderstand}.
% , We validate that the REBAR metric does in fact predict mutual class membership (i.e. $\textrm{small } d({\textbf{X}}_{anchor}, {\textbf{X}}_{\textrm{cand}})  \implies y({\textbf{X}}_{anchor})=y({\textbf{X}}_{\textrm{cand}})$). 
Thus, the REBAR metric can be used within a contrastive learning framework to identify if an anchor and a candidate should form a positive or negative pair. 

From the $i$th time-series $\textbf{A}^{(i)}$, we uniformly random sample an anchor subsequence, $\textbf{X}_{\textrm{anchor}}^{(i)}$, and $n$ candidate subsequences, $\textbf{X}_{\textrm{cand}}^{(i)}$, which make up the set $\mathcal{S}_{\textrm{cand}}^{(i)}$. Then, we can label the candidates to be the positive, $\textbf{X}_{\textrm{pos}}^{(i)}$, or to be the within-time-series negative set $\mathcal{S}_{\textrm{within-neg}}^{(i)}$. We can use these negatives with the within-time-series loss, $\mathcal{L}_w$,  modeled with NT-Xent \citep{chen2020simclr} 
\begin{align}
    \textbf{X}_{\textrm{pos}}^{(i)} &=  \underset{{\textbf{X}}_{\textrm{cand}}^{(i)} \in \mathcal{S}_{\textrm{cand}}^{(i)}}{\textrm{argmin}}  d(\textbf{X}_{\textrm{anchor}}^{(i)}, {\textbf{X}}_{\textrm{cand}}^{(i)}) \nonumber \\ % \label{eq:pos}\\ % \underset{{\textbf{X}}_{\textrm{cand}} \in \mathcal{S}_{\textrm{cand}}}{\textrm{argmin}}  \Vert\textrm{REBAR}(\bar{\textbf{X}}_{\textrm{anchor}}, {\textbf{X}}_{\textrm{cand}})-\textbf{X}_{\textrm{anchor}}\Vert_2^2 \\
    \mathcal{S}_{\textrm{within-neg}}^{(i)} &= \mathcal{S}_{\textrm{cand}}^{(i)} \setminus \{\textbf{X}_{\textrm{pos}}^{(i)}\} \nonumber % \label{eq:neg}
\end{align}


For contrastive learning, you can use any loss function, but we choose to use NT-Xent loss because its super cool and used a lot, gives us the flexibility of having multiple negatives, unlike margin-based approaches like triplet loss. With $\tau$ as temperature, NT-Xent is:



The trained REBAR cross-attention can be used to attempt to reconstruct $\bar{\textbf{X}}_{\textrm{anchor}}$ from $\textbf{X}_{\textrm{cand}}$ in which $\textbf{X}_{\textrm{anchor}}  \neq \textbf{X}_{\textrm{cand}}$. As previously discussed, the subsequent reconstruction error acts as a proxy for mutual class membership due to the motif retrieval and reconstruction properties, and it is validated empirically in Sec. \ref{sec:rebarunderstand}.
% , We validate that the REBAR metric does in fact predict mutual class membership (i.e. $\textrm{small } d({\textbf{X}}_{anchor}, {\textbf{X}}_{\textrm{cand}})  \implies y({\textbf{X}}_{anchor})=y({\textbf{X}}_{\textrm{cand}})$). 
Thus, the REBAR metric can be used within a contrastive learning framework to identify if an anchor and a candidate should form a positive or negative pair. 

From the $i$th time-series $\textbf{A}^{(i)}$, we uniformly random sample an anchor subsequence, $\textbf{X}_{\textrm{anchor}}^{(i)}$, and $n$ candidate subsequences, $\textbf{X}_{\textrm{cand}}^{(i)}$, which make up the set $\mathcal{S}_{\textrm{cand}}^{(i)}$. Then, we can label the candidates to be the positive, $\textbf{X}_{\textrm{pos}}^{(i)}$, or to be the within-time-series negative set $\mathcal{S}_{\textrm{within-neg}}^{(i)}$. We can use these negatives with the within-time-series loss, $\mathcal{L}_w$,  modeled with NT-Xent \citep{chen2020simclr} 
\begin{align}
    \textbf{X}_{\textrm{pos}}^{(i)} &=  \underset{{\textbf{X}}_{\textrm{cand}}^{(i)} \in \mathcal{S}_{\textrm{cand}}^{(i)}}{\textrm{argmin}}  d(\textbf{X}_{\textrm{anchor}}^{(i)}, {\textbf{X}}_{\textrm{cand}}^{(i)}) \nonumber \\ % \label{eq:pos}\\ % \underset{{\textbf{X}}_{\textrm{cand}} \in \mathcal{S}_{\textrm{cand}}}{\textrm{argmin}}  \Vert\textrm{REBAR}(\bar{\textbf{X}}_{\textrm{anchor}}, {\textbf{X}}_{\textrm{cand}})-\textbf{X}_{\textrm{anchor}}\Vert_2^2 \\
    \mathcal{S}_{\textrm{within-neg}}^{(i)} &= \mathcal{S}_{\textrm{cand}}^{(i)} \setminus \{\textbf{X}_{\textrm{pos}}^{(i)}\} \nonumber % \label{eq:neg}
\end{align}
\vspace{-5mm}
% \begin{align}
%     \mathcal{L}_{w}  &= \frac{\exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau)}{  \sum_{\textbf{X}_{\textrm{neg}}^{(i)} \in \mathcal{S}_{\textrm{within-neg}}^{(i)}} \exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{neg}}^{(i)}) / \tau) + \exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau) }   \label{eq:wloss}
% \end{align}
% \begin{align*}
%     \frac{\exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau)}{  \sum_{\textbf{X}_{\textrm{neg}}^{(i)} \in \mathcal{S}_{\textrm{neg}}^{(i)}} \exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{neg}}^{(i)}) / \tau) + \exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau) } 
% \end{align*}


In contrastive learning, the anchor and positive instance are pulled together and the anchor and negative instances are pushed apart in the embedding space. Due to the REBAR metric's aforementioned class-discriminative properties (which is further empircally validated in Sec. \ref{sec:rebarunderstand}), we can use REBAR to label candidate instances as being positive or negative relative to the anchor. 

The trained REBAR cross-attention can be used to attempt to reconstruct $\bar{\textbf{X}}_{\textrm{anchor}}$ from $\textbf{X}_{\textrm{cand}}$ in which $\textbf{X}_{\textrm{anchor}}  \neq \textbf{X}_{\textrm{cand}}$. Then, we can label the candidates to be the positive, $\textbf{X}_{\textrm{pos}}^{(i)}$, or to be the within-time-series negative set $\mathcal{S}_{\textrm{within-neg}}^{(i)}$. We can then use these labels in our within-time-series loss, $\mathcal{L}_w$, modeled by NT-Xent, shown below. Note that the anchor subsequence $\textbf{X}_{\textrm{anchor}}^{(i)}$ and $n$ candidate subsequences, $\textbf{X}_{\textrm{cand}}^{(i)} \in \mathcal{S}_{\textrm{cand}}^{(i)}$ are randomly sampled from the time-series $\textbf{A}^{(i)}$.
\begin{align}
    \textbf{X}_{\textrm{pos}}^{(i)} &=  \underset{{\textbf{X}}_{\textrm{cand}}^{(i)} \in \mathcal{S}_{\textrm{cand}}^{(i)}}{\textrm{argmin}}  d(\textbf{X}_{\textrm{anchor}}^{(i)}, {\textbf{X}}_{\textrm{cand}}^{(i)}) \nonumber \\ % \label{eq:pos}\\ % \underset{{\textbf{X}}_{\textrm{cand}} \in \mathcal{S}_{\textrm{cand}}}{\textrm{argmin}}  \Vert\textrm{REBAR}(\bar{\textbf{X}}_{\textrm{anchor}}, {\textbf{X}}_{\textrm{cand}})-\textbf{X}_{\textrm{anchor}}\Vert_2^2 \\
    \mathcal{S}_{\textrm{within-neg}}^{(i)} &= \mathcal{S}_{\textrm{cand}}^{(i)} \setminus \{\textbf{X}_{\textrm{pos}}^{(i)}\} \nonumber % \label{eq:neg}
\end{align}

Different loss functions could be used, but we opt to use NT-Xent loss , due to its common usage \citep{chen2020simclr, zhang2022tfc, yue2022ts2vec} and flexibility for allowing the usage of multiple negatives. We define it below:
\begin{align}
    \mathcal{L}= \frac{\exp(\cos(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau)}{  \sum_{\textbf{X}_{\textrm{neg}} \in \mathcal{S}_{\textrm{neg}}^{(i)}} \exp(\cos(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{neg}}) / \tau) + \exp(\cos(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau) } \label{eq:ntxent}
\end{align}

Now, if we define $\mathcal{S}_{\textrm{neg}} \equiv \mathcal{S}_{\textrm{within-neg}}^{(i)}$ then we would have our within-time-series loss, $\mathcal{L}_w$. This \textit{within-time-series loss captures how a time-series can change class labels over time}. It learns to pull the anchor and the subsequence that is most likely to be of the same class as the anchor, according to REBAR, together in the embedding, while pushing those that are less likely, apart. 

% This loss \textit{captures the temporally changing dynamics found within a time-series signal} by sampling subsequences from the same time-series as the anchor, and identifying the one that is most likely to be of the same class as the anchor, according to REBAR, and labeling it as positive. This loss function then pushes this pair together in the embedding space and other pairs apart. This allows us to capture the differences in class labels within a time-series, in our embedding space. 
% Our full REBAR approach is visualized in Fig. \ref{fig:rebarfull}.


Next, in order to capture the relationships between-time-series, we can also draw negatives subsequences from other time-series in our batch, $\textbf{A}^{(j)}$, where $j \neq i$, to be the between-time-series negatives set, $\mathcal{S}_{\textrm{between-neg}}$.
\begin{align}
    \mathcal{S}_{\textrm{between-neg}}^{(i)} &= \bigcup_{j \neq i } \textbf{X}_{\textrm{anchor}}^{(j)}  \nonumber
\end{align}
% \vspace{-3mm}
% \begin{align} 
%     \mathcal{L}_b  &= \frac{\exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau)}{\sum_{\textbf{X}_{\textrm{neg}}^{(j)} \in \mathcal{S}_{\textrm{between-neg}}^{(i)}} \exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{neg}}^{(j)}) / \tau) + \exp(\textrm{sim}(\textbf{X}_{\textrm{anchor}}^{(i)},  \textbf{X}_{\textrm{pos}}^{(i)}) / \tau)} \label{eq:bloss}
% \end{align}
We can now define  $\mathcal{S}_{\textrm{neg}} \equiv \mathcal{S}_{\textrm{between-neg}}^{(i)}$ for our between-time-series loss, $\mathcal{L}_b$. This \textit{between-time-series loss captures differences in time-series, as well as differences in patients}, because commonly, each time-series will originate from a different patient. This approach is most similar to augmentation-based approaches (e.g. SimCLR) that draw their negatives from the batch.



Finally, we utilize a convex combination of these two losses from Eq. \ref{eq:wloss} and \ref{eq:bloss} to create our final loss function, $\mathcal{L}$ in Eq. \ref{eq:loss}. The $\alpha$ is used to tune whether we would like to emphasize learning differences found within-timeseries or between-timeseries. For example, an accelerometry signal could emphasize learning how activity changes over time for a given user by decreasing $\alpha$, and an ECG signal could emphasize how a patient's heart condition is different from other patients by increasing $\alpha$. 
\begin{align}
    \mathcal{L} = \alpha\mathcal{L}_b + (1 - \alpha)\mathcal{L}_w \textrm{ with } 0 \leq \alpha \leq 1 \label{eq:loss}
\end{align}


\textbf{Retrieval-based Cross-Attention:} Our retrieval-based reconstruction model utilizes a cross-attention mechanism to retrieve information across different subsequences for comparison, and there are other related works that utilize cross-attention retrieval. The most common usage is for cross-modality, in which text is the query to retrieve relevant regions in an image \citep{lee2018stackedcrossattnretrieval, miech2021fastandslowcrossattnretrieval,  zheng2022crossattnretrievalcrossmodality}. Cross-attention in NLP has been used to assess semantic similarity \citep{li2020cross2self, hao2017endtoendcross} and to provide augmentations while training another model in a Q\&A task \citep{yang2020crossattnretrieval}. In time-series, cross-attention has been used to retrieve the most salient information from a signal  \citep{garg2021sdma} and to retrieve time-series to aid forecasting \citep{yang2022mqretnn}.
%  For time-series, \citep{garg2021sdma} learns a cross-attention network to use a curated saliency series to retrieve salient information, and \citep{yang2022mqretnn} utilizes cross-attention to retrieve time-series from a database to assist in forecasting.
% for NLP and is similar to our frozen REBAR cross-attention network used to train a contrastive learning encoder in a representation learning task for time-series, but the setting and learning objectives remain distinctly different. 
% We note that the Retrieval-Enhanced Transformer \citep{borgeaud2022retro} does not use the transformer for retrieval, unlike our approach with cross-attention. Instead, they use a kNN method to retrieve the most relevant documents for the transformer encoder/decoder network. 
% REBAR is a novel method that utilizes a retrieval-based method for contrastive learning. 
Although there are self-supervised works that use retrieval for evaluation \citep{chen2021deepretrieval, ma2022xclip, wang2022coder}, these are very different from REBAR, in which a retrieval-based method is used to directly train the self-supervised learning approach.



% In our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, and the REBAR metric. The specific meaning will be evident from the context.} approach, we leverage this intuition by 

% using retrieval-based reconstruction for motifs, then using the subsequent error o identify semantically meaningful relationships.

% using retrieval of motifs to identify semantically meaningful relationships
% propose to measure similarity between sequences via reconstruction accuracy achieved from 

% reconstructing a sequence from retrieved motifs from another

% REBAR reconstructs a sequence 


% builds upon this intuition with the key idea: we can use REBAR
% semantically-meaningful 

% REBAR is able to capture how semantically similar two sequences are, by masking Retrieve and reconstruct motifs

% This idea that the specific motifs within the subsequence are class-discriminative is widely-studied and validated throughout the time-series data-mining literature \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}. Therefore, two subsequences with similar motifs are likely to be semantically related and are a good candidate to form a positive pair. Our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, and the REBAR metric. The specific meaning will be evident from the context.} approach builds upon this intuition with two key ideas:

% % \vspace{-1mm}
% % \textit{Key Idea (1): We can capture motif-similarity with retrieval-based reconstruction.} Our REBAR model reconstructs a masked out anchor sequence by retrieving motifs in a candidate sequence that match the not-masked context in the anchor. \\
% % \textit{Key Idea (2): The ensuing reconstruction error captures semantic relationships, useful for guiding contrastive learning.} We illustrate this intuition in Fig. \ref{fig:intuition}. REBAR error serves as a quasi-distance metric between two sequences, and pairs with a closer distance can then form positive examples in contrastive learning. Because the pair is likely to share the same class label, then the resulting learned embedding space is likely to be class-discriminative. 

% \vspace{-1mm}
% \begin{itemize}[leftmargin=*,noitemsep,nosep,wide = 0pt]
% \item \textit{Key Idea (1): We can capture motif-similarity with retrieval-based reconstruction.} Our REBAR model reconstructs a partially-masked  anchor sequence by retrieving motifs in a candidate sequence that match the not-masked motifs in the anchor sequence. 
% \item \textit{Key Idea (2): The ensuing retrieval-based reconstruction error captures semantic relationships, useful for guiding contrastive learning.} We illustrate this intuition in Fig. \ref{fig:intuition}. REBAR error serves as a quasi-distance metric between two sequences, and pairs with a closer distance can then form positive examples in contrastive learning. Because the pair is likely to share the same class label, then the resulting learned embedding space is likely to be class-discriminative. 
% \end{itemize}

% We are able to demonstrate this by showing that the embedding space achieves SOTA classification results with both a linear probe and in clusterability evaluations.  
% REBAR demonstrates itself as an innovative method for time-series contrastive learning 


% Our REBAR method is an innovative method for time-series contrastive learning that achieves state-of-the-art performance on a diverse set of time-series. \textit{The main contributions of this work are: }
% \vspace{-1.5mm}


\begin{enumerate}[leftmargin=*,noitemsep,nosep]
\item We introduce a novel method of identifying positives and negative pairs with our REBAR metric, calculated from a convolutional cross-attention architecture that does retrieval and comparison of potential class-specific motifs between two sequences.\amnote{this is too technical/solution focused. Can we make this more of an intuition description? You don't need to tell me the technical details here, just why they're good. You can get into them later.}
\item To justify the idea that REBAR captures semantic relationships and as a prerequisite to contrastive learning, we show that the REBAR metric predicts mutual class membership\amnote{of what exactly? Subsequences? Full sequences?}.
\item Our REBAR contrastive learning approach achieves SOTA performance against a representative suite of contrastive learning methods that each utilize a different method of generating pos/neg pairs\amnote{pos/neg looks ugly.}, thus highlighting REBAR's strength in identifying meaningful pairs.\amnote{Can we give a concrete example of a success? It's a little bit abstract. Showcase your best result. How to make more exciting?}
\end{enumerate}


Our REBAR method uses an alternative approach to identify positive pairs not based on augmentation, instead using a learned metric to measure subsequence similarity. 

We can also compare this to other common temporal psuedo-distance metrics, such as Dynamic Time Warping (DTW) \citep{muller2007dtw} and MPdist \citep{gharghabi2018mpdist}. DTW is the minimum Euclidean distance between a pair of time-series under all possible temporal alignments, commonly used to measure similarity of time-series with differing speeds. MPdist measures motif similarity between two sequences by calculating the euclidean distances between all possible windows pairs. MPDist's window size is set to the same size as the receptive field of our dilated convolution in REBAR. These metrics perform poorly in our validation experiment and this is shown in Fig. \ref{fig:confusionmpdistrebar}. 

\begin{figure}[!htbp]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=.9\textwidth]{fig/mpdistdtw.png}
% \vspace{-.7cm}
\caption{MPDist completely fails to identify the true label for Sitting, Standing, and Laying within HAR. This is because it z-norms the subsequences before comparison, so the noise in the relatively flat subsequences (i.e. Sitting, Standing, Laying) is amplified \citep{de2019mpznorm}. DTW also fails to identify the baseline label as a majority of the predicted labels, and this seems to be due to singularity phenomenon \citep{jiang2020dtwsingular} with the PPG signals being noisy. Visualizations of the HAR and PPG signals can be seen in Appendix \ref{sec:datasetdetail}.
}
\label{fig:confusionmpdistrebar}
\end{center}
\vspace{-.1cm}
\end{figure}
TS2Vec is one of the current SOTA methods that learns time-stamp level representations with augmentations; TNC samples a nearby subsequence as a positive and utilizes a hyperparameter to estimate whether a faraway sample is negative; CPC contrasts future predictions; SimCLR contrasts the most common augmentations  (i.e. shifting, scaling, jittering); sliding-MSE is a simplified version of REBAR that uses a sliding MSE comparison as metric for evaluating pairwise similarity. We aim to assess how differing contrastive learning methods perform, so the encoder \citep{yue2022ts2vec} is kept as a control across all baselines. 


However, in time-series, constructing positive pairs is challenging because typical methods  is challenging because creating positive pairs via augmentations may break the original semantic meaning. We hypothesize that if we can retrieve information from one subsequence to successfully reconstruct another subsequence, then they should form a positive pair. Harnessing this intuition, we introduce our novel approach: Retrieval-Based Reconstruction (REBAR) contrastive learning. First, we utilize a convolutional cross-attention architecture to calculate the REBAR error between two different time-series. Then, through validation experiments, we show that the REBAR error is a predictor of mutual class membership, justifying our idea of using REBAR to identify positive pairs. Finally, once integrated into a contrastive learning framework, our REBAR method can learn an embedding that achieves state-of-the-art performance on downstream tasks across various modalities. 

In our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR metric. The specific meaning will be evident from the context.}  approach, we propose to measure the similarity between two subsequences by reconstructing one sequence from the retrieved motifs in the other that match the non-masked context. We illustrate the intuition of this idea in Fig. \ref{fig:intuition}. The ensuing reconstruction error is a quasi-distance metric that captures motif similarity, and pairs with a closer distance can then form positive examples in contrastive learning. Such pairs are likely to share semantic meaning, so that the resulting learned embedding space is class-discriminative. We are able to demonstrate this by showing that REBAR achieves state-of-the-art performance on a diverse set of time-series. The full REBAR approach can be seen in Fig. \ref{fig:rebarfull}, and our public code repository can be found here: \url{https://github.com/maxxu05/rebar}. 


\caption{This figure demonstrates the intuition of our REtrieval-BAsed Reconstruction (REBAR) approach. If we can successfully retrieve motifs from another subsequence to aid in reconstruction, then the two subsequences should form a positive pair in a contrastive learning framework. This is because subsequences of the same class are likely to share similar motifs for retrieval. b) shows that when Walking Subseq 1 is missing a point, a similar double peak motif can be identified from Walking Subseq 2 to achieve a good retrieval-based reconstruction. In c), the Sitting Subseq has no matching motif, leading to a poor reconstruction.}


 Our Retrieval-Based Reconstruction (REBAR) metric measures the similarity between two sequences as the reconstruction error that results from reconstructing one sequence with retrieved information from the other. Then, if the two sequences have high REBAR similarity, then we label them as a positive pair. Through validation experiments, we show that the REBAR error is a predictor of mutual class membership.Then, once integrated into a contrastive learning framework, our REBAR method can learn an embedding that achieves state-of-the-art performance on downstream tasks across various modalities. 
In our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR metric. The specific meaning will be evident from the context.}  approach, we propose to measure a non-symmetric distance between two subsequences by reconstructing one with the retrieved motifs from the other, and the motifs are retrieved based upon a learned motif similarity. We illustrate the intuition of this idea in Fig. \ref{fig:intuition}. REBAR is a quasi-distance metric that captures motif similarity, and pairs with a closer distance can then form positive examples in contrastive learning. Such pairs are likely to share semantic meaning, so that the resulting learned embedding space is class-discriminative. We are able to demonstrate this by showing that REBAR achieves state-of-the-art performance on a diverse set of time-series. The full REBAR approach can be seen in Fig. \ref{fig:rebarfull}, and our public code repository can be found here: \url{https://github.com/maxxu05/rebar}. 
After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate that match the non-masked out portions of the anchor. Then, we use these retrieved motifs to reconstruct the anchor, and the candidate that provides the lowest error is labeled as a positive example. 

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate and use them to reconstruct the anchor.

[DONE, i have two versions, see above. one is more detailed and one is more concise] <<MAX in words outline the basic approach here>>


%%that are generated from that specific activity class. This idea that the specific motifs within the subsequence are class-discriminative is widely-studied and validated throughout the time-series data-mining literature \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}. An obvious motif is the 3 deflections that describe a QRS complex found within an ECG signal, which directly measures the heart's depolarization \citep{bouaziz2014qrs}. A more subtle motif could be a hand-to-mouth gesture found within a wrist-based accelerometry signal, used to detect a smoking event \citep{2020chatterjeesmokingopp}. Therefore, two subsequences with similar motifs are likely to be semantically related and are a good candidate to form a positive pair. 

In our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR metric. The specific meaning will be evident from the context.}  approach, we propose to measure a non-symmetric distance between two subsequences by reconstructing one with the retrieved motifs from the other, and the motifs are retrieved based upon a learned motif similarity. We illustrate the intuition of this idea in Fig. \ref{fig:intuition}. REBAR is a quasi-distance metric that captures motif similarity, and pairs with a closer distance can then form positive examples in contrastive learning. Such pairs are likely to share semantic meaning, so that the resulting learned embedding space is class-discriminative. We are able to demonstrate this by showing that REBAR achieves state-of-the-art performance on a diverse set of time-series. The full REBAR approach can be seen in Fig. \ref{fig:rebarfull}, and our public code repository can be found here: \url{https://github.com/maxxu05/rebar}.


and a set of candidate subsequences



In REBAR, we propose to measure a non-symmetric distance between two subsequences by reconstructing one with the retrieved motifs from the other, and the motifs are retrieved based upon a learned motif similarity. We illustrate the intuition of this idea in Fig. \ref{fig:intuition}. 


Therefore, REBAR is a quasi-distance metric that captures motif similarity, and we can use it to form positive examples in contrastive learning. Specifically, after randomly sampling an anchor subsequence and a set of candidate subsequences, the candidate that helped provided the lowest REBAR error in reconstructing a masked-out anchor




we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate that match the non-masked out portions of the anchor. Then, we use these retrieved motifs to reconstruct the anchor, and the candidate that provides the lowest error is labeled as a positive example. 

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate and use them to reconstruct the anchor.

[DONE, i have two versions, see above. one is more detailed and one is more concise] <<MAX in words outline the basic approach here>>


%%that are generated from that specific activity class. This idea that the specific motifs within the subsequence are class-discriminative is widely-studied and validated throughout the time-series data-mining literature \citep{yeh2018time, yeh2016matrix, alaee2021time, li2021time}. An obvious motif is the 3 deflections that describe a QRS complex found within an ECG signal, which directly measures the heart's depolarization \citep{bouaziz2014qrs}. A more subtle motif could be a hand-to-mouth gesture found within a wrist-based accelerometry signal, used to detect a smoking event \citep{2020chatterjeesmokingopp}. Therefore, two subsequences with similar motifs are likely to be semantically related and are a good candidate to form a positive pair. 

 Such pairs are likely to share semantic meaning, so that the resulting learned embedding space is class-discriminative. 


We are able to demonstrate this by showing that REBAR achieves state-of-the-art performance on a diverse set of time-series. The full REBAR approach can be seen in Fig. \ref{fig:rebarfull}, and our public code repository can be found here: \url{https://github.com/maxxu05/rebar}. 




Given a partially-masked subsequence A and another subsequence B, we can reconstruct A by identifying motifs in B that match the non-masked motifs of A, and then using these motifs from B to reconstruct A.

viewpoint matching in vision, but they arent really related in some similar comparison
motifs are stable, "Anchors" and garbage is not

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate that match the non-masked out portions of the anchor. Then, we use these retrieved motifs to reconstruct the anchor, and the candidate that provides the lowest error is labeled as a positive example. 






We use motif-similarity to identify regions in which 

We have one motif in the query and 

We use a motif to query motifs in the key to find a motif match. once we find a match, we can use this motif to attempt to reconstruct the original.

We learn a retrieval function that 

Why are we doing this instead of just regular motif-matching?

We learn a retrieval function that identifes matching motifs that would be useful for reconstruction

We learn a motif-matching function with a reconstruction objective that retrieves matching motifs 


model can only reconstruct as;dlfkj




In our REBAR approach, we reconstruct one sequence by retrieving information from another, and the information retrieved is based upon a learned motif-similarity.

Essentially, if sequence A has similar motifs as sequence B, then we can query sequence B for 


we want to reconstruct sequence A, but can only fill in the missingness 

but the information that is being used to reconstruct A, must be derived from the other sequence B. 



can capture motif-similarity between sequence A and B by doing a motif similarity comparison fbetween A and B and then using the motifs similar to A to be used to reconstruct A

In our REBAR approach, we learn a retrieval function that identifies motifs in sequence A that matches motifs in B. Then we can use the identified motifs in sequence A to reconstruct a masked out sequence B.

In our REBAR approach, we use a reconstruction objective function with a convolutional cross-attention model that learns motif-similarity, in order to retrieve motifs for reconstruction.

In our REBAR, we have a psuedo-distance metric between a sequence A and sequence B

In our REBAR approach, we have two sequences, sequence A we designate as being partially masked, and sequence B, which is  signal is partially masked and the other 

We learn a motif-similarity function based on 

1) query other signal for useful motifs
2) retrieve most useful motifs for reconstruct 

Then, we can use REBAR cross-attention


we reconstruct a signal A by using signal A to query 

we query signal B for motifs that match the signal A, and then we use matching motifs in B to reconstruct A


we learn cross-attention that learns how to compare motifs, 



learn how to identify motifs in B that are the most similar to the motifs in A to be retrieved to fill in gaps in A.


65

we learn a reconstruction that only works via motif retrieval. then the motif retrieval captures motif similarity


propose to measure the distance from sequence A to sequence B 


Given two sequences, A and B, we can use 
We would like to use to use sequence B to reconstruct sequence A. 
During reconstruction of sequence A

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate that match the non-masked out portions of the anchor. Then, we use these retrieved motifs to reconstruct the anchor, and the candidate that provides the lowest error is labeled as a positive example. 

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate and use them to reconstruct the anchor.

[DONE, i have two versions, see above. one is more detailed and one is more concise. the ideas of the basic outline are in the next paragraph too though. they tell similar stories but ] <<MAX in words outline the basic approach here>>

Classical approaches based upon motif mining can involve specific domain expertise or brute-force all-pair comparisons from fixed size windows. 
While one could imagine approaches to subsequence matching that try to explicitly model and compare motifs, classical approaches based on motif mining are computationally expensive, and can't be trained to produce a similarity measure which is adapted to a particular domain of data (like ECG). The ability to train a measure makes it possible to leverage the temporal structure of a domain of data, and its computationally feasible because the cost of learning is amortized over many rounds of testing (where the learned measure is used to construct minibatches for conntrastive learning).

Our key idea is to turn this around and rather than focusing on identifying and matchinig motifs explicitly, we exploit the fact that a deep model can learn to use motifs implicitly in a reconstruction task. Suppose we are computing the correspondence between a source subsequence A and a target subsequence B. Suppose we pick a random set of samples in A and mask them out, and then attempt to reconstruct the masked samples using the samples from sequence B. This can be accomplished by defining a context window around each masked sample, finding the best match for that signal context in B, and then filling in the missing sample given the best match. We train the REBAR architecture to take a context window with a masked sample as an input, along with sequence B, and output the missing sample through a purely feed-forward process. Since the REBAR model is trained to perform this reconstruction task, it learns which features within the time series subsequence are stable and meaningful and can be used to match the context window to the most similar portion of sequence B. In particular, the model can learn an appropriate receptive field size in B which can adapt to the data domain and vary with the query, providing significant flexibility in comparing the two subsequences.

We operationalize the idea of matching motifs through our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR metric. The specific meaning will be evident from the context.} approach. Rather than identifying motifs explicitly, we exploit the fact that a deep model can learn to use motifs implicitly in a reconstruction task. Assume we are computing the similarity between subsequence A and a subsequence B. After masking out a set of random time-point in A, we can take a context window around each of the masked point to be compared to windows in B. Our REBAR cross-attention model can then compare motifs within these windows to retrieve matching motifs from B to be used to reconstruct A. Then, the REBAR reconstruction error is a learned measure that captures motif similarity, and pairs with a lower error can then form positive examples in contrastive learning. 

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate that match the non-masked out portions of the anchor. Then, we use these retrieved motifs to reconstruct the anchor, and the candidate that provides the lowest error is labeled as a positive example. 

After sampling an anchor subsequence and a set of candidate subsequences at random, we mask out the anchor and then use a learned motif-similarity retrieval function to retrieve motifs from the candidate and use them to reconstruct the anchor.


Given a partially-masked subsequence A and another subsequence B, we can reconstruct A by using the non-masked motifs of A to query for similar motifs in B, and then using these motifs to reconstruct A. In this way, we can measure a non-symmetric distance between two subsequences by reconstructing one subsequence from the retrieved motifs from the other.


In our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR metric. The specific meaning will be evident from the context.}  approach, we propose to measure a non-symmetric distance between two subsequences by reconstructing one with the retrieved motifs from the other, and the motifs are retrieved based upon a learned motif similarity.

EBAR is a quasi-distance metric that captures motif similarity, and pairs with a closer distance can then form positive examples in contrastive learning. Such pairs are likely to share semantic meaning, so that the resulting learned embedding space is class-discriminative. We are able to demonstrate this by showing that REBAR achieves state-of-the-art performance on a diverse set of time-series. The full REBAR approach can be seen in Fig. \ref{fig:rebarfull}, and our public code repository can be found here: \url{https://github.com/maxxu05/rebar}. 


We operationalize the idea of matching motifs with our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR measure. The specific meaning will be evident from the context.} approach by using a deep model to learn how to use motifs implicitly during reconstruction. Assume we are computing the similarity between subsequence A and a subsequence B. After masking out a set of random time-point in A, we can take a context window around each of the masked points to compare them to windows in B. We illustrate the intuition of this idea in Fig. \ref{fig:intuition}. Our REBAR cross-attention model compares motifs within these windows to retrieve matching motifs from B to be used to reconstruct A. Then, the REBAR reconstruction error is a learned measure that captures motif similarity, and pairs with a lower error can then form positive examples in contrastive learning. Such pairs are likely to share semantic meaning, so that the resulting learned embedding space is class-discriminative. We are able to demonstrate this by showing that REBAR achieves state-of-the-art performance on a diverse set of time-series. The full REBAR approach can be seen in Fig. \ref{fig:rebarfull}, and our public code repository can be found here: \url{https://github.com/maxxu05/rebar}. 


We operationalize the idea of matching motifs with our Retrieval-Based Reconstruction (REBAR)\footnote{Note that we will interchangeably use "REBAR" to refer to the REBAR contrastive learning approach, the REBAR cross-attention, or the REBAR measure. The specific meaning will be evident from the context.} approach. In order to avoid explicitly modeling and detecting motifs, we adopt a reconstruction-based approach in which  masked samples in one subsequence are reconstructed from corresponding values in a second subsequence, as illustrated in Fig. \ref{fig:intuition}. Each masked sample is at the center of a context window, and the trained model learns to match each context window to corresponding samples in the target subsequence in order to minimize the reconstruction error. When two subsequences have many motifs in common, high quality matches can be obtained that minimize the error. This approach has the advantage of simplicity: reconstruction error on a sparse set of masked samples can be used to train a single feedforward model that can reconstruct them simultaneously. At the same time, the receptive field that defines how the target sequence is analyzed is learned during training, allowing the model to adapt to the statistical properties of the time series data.



